THOR: A Non-Speculative Value Dependent Timing Side Channel Attack Exploiting Intel AMX

The rise of on-chip accelerators signifies a major shift in computing, driven by the growing demands of artificial intelligence (AI) and specialized applications. These accelerators have gained popularity due to their ability to substantially boost performance, cut energy usage, lower total cost of ownership (TCO), and promote sustainability. Intel's Advanced Matrix Extensions (AMX) is one such on-chip accelerator, specifically designed for handling tasks involving large matrix multiplications commonly used in machine learning (ML) models, image processing, and other computational-heavy operations. In this paper, we introduce a novel value-dependent timing side-channel vulnerability in Intel AMX. By exploiting this weakness, we demonstrate a software-based, value-dependent timing side-channel attack capable of inferring the sparsity of neural network weights without requiring any knowledge of the confidence score, privileged access or physical proximity. Our attack method can fully recover the sparsity of weights assigned to 64 input elements within 50 minutes, which is 631% faster than the maximum leakage rate achieved in the Hertzbleed attack.

==> Shorts/Intro-short.tex <==
 \section{Introduction}



==> Table_Thor.tex <==
% Add extra row height
\setlength{\extrarowheight}{2pt}

%\vspace{1cm}
\hspace*{0.6cm}  % Move the table to the left if needed
\scalebox{0.3}{ % Adjust the scaling factor as needed
\begin{tabular}{C|X|P@{}P@{}P@{}P@{}P@{}P@{}P@{}P@{}P@{}P@{}P@{}P@{}P@{}P@{}P@{}C@{\hspace{1.2cm}}}
\textbf{Category} & \diagbox[width=3.8cm,height=1.5cm]{\textbf{Attack}}{\textbf{Defense}}
& \makebox[1.2cm][c]{\smash{\raisebox{0.1cm}{\rotatebox{45}{\textbf{Fence}}}}}
& \makebox[2cm][c]{\smash{\raisebox{0.1cm}{\rotatebox{45}{\textbf{Invisispec}}}}}
& \makebox[1.8cm][c]{\smash{\raisebox{0.1cm}{\rotatebox{45}{\textbf{DAWG}}}}}
& \makebox[2.5cm][c]{\smash{\raisebox{0.1cm}{\rotatebox{45}{\textbf{Taint Tracking}}}}}
& \makebox[3cm][c]{\smash{\raisebox{0.1cm}{\rotatebox{45}{\textbf{Timer Coarsening}}}}}
& \makebox[2cm][c]{\smash{\raisebox{0.1cm}{\rotatebox{45}{\textbf{IBPB}}}}}
& \makebox[2.2cm][c]{\smash{\raisebox{0.1cm}{\rotatebox{45}{\textbf{Retpoline}}}}}
& \makebox[2.5cm][c]{\smash{\raisebox{0.1cm}{\rotatebox{45}{\textbf{SSBD/SSB}}}}}
& \makebox[2.5cm][c]{\smash{\raisebox{0.1cm}{\rotatebox{45}{\textbf{KPTI}}}}}
& \makebox[5.2cm][c]{\smash{\raisebox{0.1cm}{\rotatebox{45}{\textbf{Disabling-DVFS}}}}}
& \makebox[5.3cm][c]{\smash{\raisebox{0.1cm}{\rotatebox{45}{\textbf{Disabling SMT}}}}}
& \makebox[6.3cm][c]{\smash{\raisebox{0.1cm}{\rotatebox{45}{\textbf{Making RAPL Privileged}}}}}
& \makebox[4.8cm][c]{\smash{\raisebox{0.1cm}{\rotatebox{45}{\textbf{Masking}}}}} 
& \makebox[6.7cm][c]{\smash{\raisebox{0.1cm}{\rotatebox{45}{\textbf{Restrict Physical Access}}}}}
& \makebox[5.3cm][c]{\smash{\raisebox{0.1cm}{\rotatebox{45}{\textbf{ EM Defense}}}}}
& \makebox[6cm][c]{\smash{\raisebox{0.1cm}{\rotatebox{0}{\textbf{Target}}}}}\\
\hline
\end{tabular}}
\hspace*{-0.33cm}  % Move the table to the left if needed
\scalebox{0.3}{ % Adjust the scaling factor as needed
\begin{tabular}{|C|X|P@{}P@{}P@{}P@{}P@{}:P@{}P@{}@{}P:P@{}:@{}P@{}P@{}P:@{}P@{}P@{}P|C|}
\multirow{2}{*}{\textbf{Transient}} & \textbf{Spectre} & \fullcircle & \fullcircle & \fullcircle & \fullcircle & \fullcircle & \halfcircle & \halfcircle & \fullcircle & \emptycircle & \emptycircle & \emptycircle & \emptycircle & \emptycircle &\emptycircle &\emptycircle\\
& \textbf{Meltdown} & \fullcircle & \emptycircle & \fullcircle & \fullcircle & \fullcircle & \emptycircle & \emptycircle & \emptycircle & \fullcircle & \emptycircle & \emptycircle  & \emptycircle & \emptycircle &\emptycircle &\emptycircle\\
\hline
\multirow{2}{*}{\textbf{MDS}} & \textbf{LVI} & \fullcircle & \emptycircle & \emptycircle & \emptycircle & \fullcircle & \emptycircle & \emptycircle & \emptycircle & \emptycircle & \emptycircle & \fullcircle & \emptycircle & \emptycircle &\emptycircle &\emptycircle\\
& \textbf{Fallout} & \fullcircle &\emptycircle &\emptycircle &\emptycircle &\fullcircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle\\
& \textbf{Downfall} & \fullcircle &\emptycircle &\emptycircle &\emptycircle &\fullcircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle & \fullcircle &\emptycircle &\emptycircle &\emptycircle\\
\hline
\multirow{1}{*}{\textbf{Frequency}} & \textbf{Hertzbleed} &\emptycircle &\emptycircle &\emptycircle &\emptycircle & \fullcircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle & \fullcircle & \emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle\\
\hline
\multirow{3}{*}{\textbf{Power}} & \textbf{Collide+Power\_v1}  &\emptycircle &\emptycircle &\fullcircle &\emptycircle &\fullcircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\halfcircle &\emptycircle & \halfcircle &\emptycircle &\emptycircle &\emptycircle\\
& \textbf{Collide+Power\_v2} &\emptycircle &\emptycircle &\fullcircle &\emptycircle &\fullcircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle & \halfcircle & \fullcircle & \halfcircle &\emptycircle &\emptycircle &\emptycircle\\
& \textbf{Platypus} &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle & \fullcircle &\emptycircle &\emptycircle &\emptycircle\\
\end{tabular}}
\hspace*{0.7cm}
\scalebox{0.3}{ % Adjust the scaling factor as needed
\begin{tabular}{|C|X|P@{}P@{}P@{}P@{}P@{}:P@{}P@{}@{}P:P@{}:@{}P@{}P@{}P:@{}P@{}P@{}P|C|}
\hline
\multirow{7}{*}{\textbf{Neural}} & \textbf{Cache Telepathy, GANRED, DeepRecon} & \emptycircle & \emptycircle & \fullcircle & \emptycircle & \fullcircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &NN Arch\\
\cdashline{2-18}
& \textbf{DeepEM, DeepSniffer} &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\fullcircle &\fullcircle &NN-Arch\\
\cdashline{2-18}
& \textbf{Open DNN Box} &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\fullcircle &\emptycircle &weight-sparsity\\
\cdashline{2-18}
& \textbf{CSI NN} &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\fullcircle &\fullcircle &weight/arch\\
\cdashline {2-18}
& \textbf{I Know What You See} &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle & \fullcircle &\fullcircle &\emptycircle &NN-inputs\\
\cdashline{2-18}
& \textbf{Reverse-Engineering DNNs} &\emptycircle &\emptycircle &\halfcircle &\emptycircle &\fullcircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle & \emptycircle &\halfcircle &\emptycircle &Model-Params\\
\cdashline{2-18}
& \textbf{Thor} &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\fullcircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &\emptycircle &NN-weights\\
\hline
\end{tabular}}


==> contents/Alg.tex <==
\begin{algorithm}[!bp]
\caption{ Zero Value Inference through Intel AMX Execution Time Analysis}
{\footnotesize\begin{algorithmic}[1]
\Statex \textbf{Definitions:}
\Statex \( P1 \) - The network processes for \( N \) iterations.
\Statex \( P2 \) - The execution of \( P1 \) followed by a cooling-down delay (20 ms).
\Statex \( P3 \) - Repeated execution of \( P2 \) for  \( M \) iterations.
\Statex \( T \) - The execution time of \( P3 \), excluding the cooling-down delays.
\Statex \( ScoreZ \) - A score vector where each element corresponds to the likelihood of a weight being zero.
\Statex \( ScoreN \) - A score vector where each element corresponds to the likelihood of a weight being non-zero.
\Statex \( W_{\text{Out}} \) - Final estimated weight values.

\Statex \textbf{Procedure:}
\State $T_Z \gets \text{Fill the input with zeros and measure \( T \).}$
\State $T_N \gets \text{Fill the input with non-zeros and measure \( T \).}$
\State $T_d \gets T_N - T_Z$
\State $T_m \gets$ Perform steps 1 to 3 multiple times (\(L\) iterations), calculating the average of the largest \(K\) values of \(T_d\).
\State $Thr \gets \text{Set a threshold equal to } \alpha \times T_m.$
\State Generate a random vector (\( W_s \)), and use it as network input.
\State $T_s \gets \text{measure \( T \).}$
\State Invert \( W_s \) (switch all zeros to non-zeros and all non-zeros to zeros) to create \( W_r \), then use \( W_r \) as network input.
\State $T_r \gets \text{measure \( T \).}$
\State \textbf{if } (\(|T_s - T_r| > Thr\)) \textbf{then} 
\State \quad \textbf{if } (\(T_s > T_r\)) \textbf{then} 
\State \quad \quad $W_x \gets W_s$
\State \quad \textbf{else}
\State \quad \quad $W_x \gets W_r$
\State \quad \textbf{end}
\State \quad \textbf{for } $i \gets$ 0 to 63 \textbf{do} 
\State \quad \quad \textbf{if } (\(W_x[i] == 0\)) \textbf{then} 
\State \quad \quad \quad $ScoreZ[i] \gets ScoreZ[i]+1$
\State \quad \quad \textbf{else }
\State \quad \quad \quad $ScoreN[i] \gets ScoreN[i]+1$
\State \quad \quad \textbf{end}
\State \quad \textbf{end}
\State \textbf{end}
\State Repeat steps 6 to 23 over the attack duration.
\State \textbf{for } $i \gets$ 0 to 63 \textbf{do} 
\State \quad \textbf{if } (\(ScoreN[i]/ScoreZ[i] > \gamma\)) \textbf{then} 
\State \quad \quad \( W_{\text{Out}}[i] \) $\gets non-zero$
\State \quad \textbf{else }
\State \quad \quad \( W_{\text{Out}}[i] \) $\gets zero$
\State \quad \textbf{end}
\State \textbf{end}
\end{algorithmic}}
\label{alg:alg1}
\end{algorithm}

==> contents/Background.tex <==
% %\notema{add some intro words here}

% % In this section, we present a background on related micro-architectural attacks, an overview of built-in accelerators and their benefits, as well as a background on Intel AMX instruction and architecture.  


% %\subsection{Microarchitectural Side-channel Attacks}
% %\{Overview of side-channel attacks, defining covert channel, leakage gadget, etc?}\SMA{ to : No we don't need to explain those.There won't be space.} 
% %\SMA{For each attack, add their threat model and parameters that matter to CVSS, such as scope, vector,  complexity, and information that would build context around **your paper's findings**. To help them better appreciate your findings. Not to teach a whole Wikipedia in half a page. }
% %\subsubsection{Cache attacks}
% %The oldest side-channel attacks are cache attacks. 
% %\notema{this section requires some more polishing}
% %\notema{osvik: Cache Attacks and Countermeasures: the Case of AES. should be cited as well for prime+probe}

% % \begin{figure}[!t]
% %     \centering
% %    \includegraphics[width=\linewidth]{images/AMXarch_new_v1.pdf} 
% %     \caption{Intel AMX Architecture Overview}
% %     \label{fig:AMX-arch}
% % \end{figure}

% % \textbf{{Intel AMX Architecture and Instructions.}}
% % Intel AMX is an integrated accelerator introduced with the 4th Gen Intel Xeon Scalable processors, specifically engineered to boost the efficiency of matrix computations that are essential for artificial intelligence and high-performance computing applications. Figure~\ref{fig:AMX-arch} illustrates the Intel AMX architecture.

% % AMX introduces a new set of registers and instructions. The registers in Intel AMX are known as Tiles, a new concept in Intel CPUs that provide a matrix of data registers, as opposed to the traditional vector registers seen in previous SIMD architectures like AVX-512. AMX includes 8 Tile registers, each capable of holding up to 16 rows with 64 bytes per row, amounting to a total of 1 KB per Tile. The number of rows and the number of bytes per row can be adjusted using the LDTILECFG instruction, and this configuration information is stored as metadata in a control register known as TILECFG. Once this configuration is set, AMX instructions such as load, store, and matrix multiplication will operate according to the specified dimensions for each Tile. Intel AMX instructions are synchronized with the Intel Architecture host (IA host) instruction stream, and the Tile loads and stores are coherent with the host memory \cite{Intel_Arc_Ins_Set_Extensions}.

% % Tile Matrix Multiply unit (TMUL) serves as the accelerator engine for executing multiplication calculations. When using full-size Tile operands, the latency of the multiplication instruction is 52 cycles, while pipelining allows for a throughput of 16 cycles. Intel AMX supports two data types: BF16 and INT8. Consequently, it can perform 512 multiplications and 512 additions per cycle for BF16 and 1024 multiplications and 1024 additions per cycle for INT8 \cite{IntelOptRefManual}. 

% % AMX instructions utilize port 5 as their dedicated execution port. When two hyper-threads are active within a core, they compete for the same resources to execute AMX instructions.


% \paragrabf{Cache attacks.}
% Cache attacks exploit timing differences caused by loading data from different cache levels or the DRAM.
% In \PrimeProbe~\cite{prime_probe,osvik2006cache}, the attacker "primes" a cache set and waits for the victim to execute, tracking evictions. Flush+Reload \cite{flush+reload} flushes a cache line and checks if it was filled by the victim.
% % Flush+Reload \cite{flush+reload} 
% % uses the presence or absence of a variable shared between the attacker and victim (e.g. in a shared library) to deduce a victim's program path.
% Flush+Flush attack ~\cite{GrussFlushFlush} relies on the execution time variation of the flush instruction.

% %\subsubsection{Speculative \& Transient Attacks} 

% \paragrabf{Transient-execution attacks.}
% % Spectre \cite{kocher2020spectre}
% %is a class of attacks that abuse mechanisms that result in jumps in code (e.g. branch predictor, pattern history table) to speculatively execute certain instructions that have a measurable effect on the microarchitecture (but not the architecture). For example, in Spectre-v1
% % %\notema{Use the classification of Canella et al} 
% % the branch predictor is mistrained on a particular branch with a value that points to an in-bound variable. The attacker then changes the value to point to an out-of-bounds and causes the branch to execute. Due to out-of-order execution, for a small amount of cycles the incorrect code can execute which, when the measurable microarchitectural change caused by the code is dependent on the out-of-bounds value, can lead to an attacker being able to read the entirety of a process's address space. Other attacks include 
% % and Meltdown 
% % \cite{meltdown};
% Spectre \cite{kocher2020spectre} exploits speculative execution of an operation that would not occur during correct execution path of the program. Meltdown-type attacks \cite{meltdown} exploit delayed
% exception handling during out-of-order execution.
% % e.g. there was a null pointer access but the check for the exception was executed after other transient instructions were being executed.
% Forshadow~\cite{van2018foreshadow}
% %\notema{what about foreshadow?} 
% exploits a bug in Intel CPUs that led to imperfect isolation of the SGX enclave context, Load Value Injection \cite{lvi} induces execution based on malicious values injected in various microarchitectural buffers, Fallout \cite{canella2019fallout} leaks the contents of the store buffer, and RIDL \cite{ridl} and Zombieload \cite{schwarz2019zombieload} leak the contents of the line fill buffer.


% \paragrabf{Software-based power side-channel attacks.}
% %\subsubsection{Software Power Side channel attacks like Platypus}
% Platypus \cite{Lipp2021Platypus} exploits the RAPL (Running Average Power Limit) driver, to infer the internal state of a program, even inside an SGX enclave. This vulnerability was mitigated by kernel updates restricting RAPL access and Intel microcode updates changing how power is reported in the context of SGX.
% %for everything except SGX 
% % by restricting RAPL access to privileged users using a kernel update and was mitigated for privileged users through an Intel microcode update that decorrelated the power report from operands in the context of an SGX enclave. 
% %\{This is wrong. Intel released a microcode update that changes how power is reported when in the context of an SGX enclave}. \SMA{Who wrote that? Martin?  it seems like someone wrote that was confident. Ohhh I see this is right because with malicious OS, OS has access to RAPL? But Micro code fixed it. So don't say that if we are not sure. }
% Collide+Power~\cite{kogler2023collide+} uses a differential power measurement technique involving pairs of inputs with their inverses to leak victim data coexisting with attacker data in the same microarchitectural buffers. 
% %\subsubsection{Attacks that exploit accelerators}
% % Grand Pwning Unit \cite{frigo2018grand} explored using GPUs to accelerate microarchitectural attacks, specifically RowHammer\notema{Not sure if Rowhammer and GPUs are relevant here..}. They found that since the GPU is accessible from Javascript, it is possible to mount a Rowhammer attack by injecting Javascript code into a web browser. 



% %\subsubsection{Remote attacks}
% % \paragrabf{Remote timing attacks.}
% % Many remote side-channel attacks were solely focusing on cryptographic primitives such as AES or RSA ~\cite{Aciicmez2007d,Brumley2003Remote,Bernstein2005,Zhao2009cache,Jayasinghe2010remote,Aly2013attacking,Saraswat2014}.
% % Irazoqui \etal\cite{Irazoqui2015Lucky} attacked TLS in a remote setup leveraging cache timing differences.
% % Schwarz \etal\cite{schwarz2019netspectre} demonstrated Spectre attacks in a fully remote setup (with controlled network traffic) leveraging both a cache side channel and an AVX side channel to remotely exfiltrate data.
% % \cite{VanGoethem2020Timeless} makes use of the relative timing difference in response time to tackle existing jitter in networks. 
% % Moreover, remote attacks were created leaking data by exploiting operating system optimizations ~\cite{Gruss2019page,Schwarzl2022Remote}, DVFS to attack post-quantum cryptography~\cite{wang2022hertzbleed} and the compression ratio~\cite{schwarzl2023practical}.
% % %Memory compression attacks work only on programs that employ memory compression like web servers; Loki is more general than this functioning on any program that listens for network requests and utilizes the AMX unit. Hertzbleed relies on dynamic voltage and frequency (DVFS) scaling while Loki works independently of DVFS.

% % %\SMA{The immediate  question comes in mind is why we didn't compare with all of these? Are they out of scope? Are they about something else? What is common what is not common. This section without a conclusion in comparison with our work kills our paper. Our paper gets killed without having it as well. Justify. TODO . Also after reading it it feels like our work is not novel so for example say, "Although these works studied remote attacks in this and that condition but they didn't study this or couldnt do that or their impact was weak... on the other hand we .... the comparison with Netspectre and blah blah is given in section blah"}

% % \noindent\textbf{{Signal Amplification.}}
% % Amplifying a side channel's signal strength, e.g. the timing difference, can significantly reduce noise.
% % Roettger and Janc~\cite{Roettger2021A} leveraged the PLRU cache replacement policy in the L1 to arbitrarily amplify a single cache hit. However, it relies on the cache and thus any cache side-channel defense, e.g.\ \cite{Invisispec}, would mitigate this issue. Additionally, this method may be detectable in hardware.
% % Hacky Racers~\cite{HackyRacers2023ASPLOS} %introduced "racing gadgets" and "magnifier gadgets" by exploiting 
% % exploited instruction-level parallelism enabling timing attacks on restricted system such as JavaScript, although, multiple execution of the "magnifier gadget" in this paper makes it detectable in hardware.  MicroScope \cite{Microscope} addresses the issue of noisy side-channels, which mandates multiple measurements for getting reliable data by utilizing core microarchitectural features to execute dynamic instruction more than once. However, this attack is detectable in hardware, as shown in \cite{EVAX2022Micro,PerSpectron}. Recent papers have enabled performing logical operation on cache signals and amplifying them to the extent that they are visible to even coarse timers, compromising the performance of the attack because of the amplification overhead~\cite{kaplan2023optimization, purnal2023showtime, katzman2023gates}. 
% % %\SMA{ , What are the weaknesses in these papers, check leakage rate, accuracy complexity requirement?Why Loki matters when these magnifiers exists}

% \textbf{{Side-channel attacks that leak ML parameters.}}
% Wei et al. \cite{wei2018know} were able to reconstruct the user inputs only by knowing the structure of the underlying CNN through measuring the power profile. Similarly, \cite{zhang2021stealing, tian2021remote} extracted neural network structure from FPGA using power side-channels.
% \cite{dubey2020maskednet}, uses differential power analysis to extract parameters of a NN.

% % {This paragraph needs review. (Not well written.)}

% % \SMA{I agree,  it shouldn't be only about what it leaks (Impact) for example Forshadow leaks kernel, it should be about their method Key idea/root cause of vulnerability and also Impact.}
% % \notema{canella defined a difference between spectre and meltdown - spectre exploits mispredictions by the branch predictor leading to transient accesses while for meltdown-type effects the underlying root cause is delayed
% % exception handling during out-of-order execution. e.g. there was a null pointer access but the check for the exception was executed after other transient instructions were being executed.}

% % %\subsubsection{Rowhammer}
% % \paragrabf{Software-based power side-channel attacks.}
% % %\subsubsection{Software Power Side channel attacks like Platypus}
% % Platypus \cite{Lipp2021Platypus} exploits the RAPL (Running Average Power Limit) driver, to infer the internal state of a program, even inside an SGX enclave. This vulnerability was mitigated by kernel updates restricting RAPL access and Intel microcode updates changing how power is reported in the context of SGX.
% % %for everything except SGX 
% % % by restricting RAPL access to privileged users using a kernel update and was mitigated for privileged users through an Intel microcode update that decorrelated the power report from operands in the context of an SGX enclave. 
% % %\{This is wrong. Intel released a microcode update that changes how power is reported when in the context of an SGX enclave}. \SMA{Who wrote that? Martin?  it seems like someone wrote that was confident. Ohhh I see this is right because with malicious OS, OS has access to RAPL? But Micro code fixed it. So don't say that if we are not sure. }
% % Collide+Power~\cite{kogler2023collide+} uses a differential power measurement technique involving pairs of inputs with their inverses to leak victim data coexisting with attacker data in the same microarchitectural buffers. 
% % %\subsubsection{Attacks that exploit accelerators}
% % % Grand Pwning Unit \cite{frigo2018grand} explored using GPUs to accelerate microarchitectural attacks, specifically RowHammer\notema{Not sure if Rowhammer and GPUs are relevant here..}. They found that since the GPU is accessible from Javascript, it is possible to mount a Rowhammer attack by injecting Javascript code into a web browser. 



% % %\subsubsection{Remote attacks}
% % \paragrabf{Remote timing attacks.}
% % Many remote side-channel attacks were solely focusing on cryptographic primitives such as AES or RSA ~\cite{Aciicmez2007d,Brumley2003Remote,Bernstein2005,Zhao2009cache,Jayasinghe2010remote,Aly2013attacking,Saraswat2014}.
% % Irazoqui \etal\cite{Irazoqui2015Lucky} attacked TLS in a remote setup leveraging cache timing differences.
% % Schwarz \etal\cite{schwarz2019netspectre} demonstrated Spectre attacks in a fully remote setup (with controlled network traffic) leveraging both a cache side channel and an AVX side channel to remotely exfiltrate data.
% % \cite{VanGoethem2020Timeless} makes use of the relative timing difference in response time to tackle existing jitter in networks. 
% % Moreover, remote attacks were created leaking data by exploiting operating system optimizations ~\cite{Gruss2019page,Schwarzl2022Remote}, DVFS to attack post-quantum cryptography~\cite{wang2022hertzbleed} and the compression ratio~\cite{schwarzl2023practical}.
% % %Memory compression attacks work only on programs that employ memory compression like web servers; Loki is more general than this functioning on any program that listens for network requests and utilizes the AMX unit. Hertzbleed relies on dynamic voltage and frequency (DVFS) scaling while Loki works independently of DVFS.

% % %\SMA{The immediate  question comes in mind is why we didn't compare with all of these? Are they out of scope? Are they about something else? What is common what is not common. This section without a conclusion in comparison with our work kills our paper. Our paper gets killed without having it as well. Justify. TODO . Also after reading it it feels like our work is not novel so for example say, "Although these works studied remote attacks in this and that condition but they didn't study this or couldnt do that or their impact was weak... on the other hand we .... the comparison with Netspectre and blah blah is given in section blah"}

% % \textbf{{Signal Amplification.}}
% % Amplifying a side channel's signal strength, e.g. the timing difference, can significantly reduce noise.
% % Roettger and Janc~\cite{Roettger2021A} leveraged the PLRU cache replacement policy in the L1 to arbitrarily amplify a single cache hit. However, it relies on the cache and thus any cache side-channel defense, e.g.\ \cite{Invisispec}, would mitigate this issue. Additionally, this method may be detectable in hardware.
% % Hacky Racers~\cite{HackyRacers2023ASPLOS} %introduced "racing gadgets" and "magnifier gadgets" by exploiting 
% % exploited instruction-level parallelism enabling timing attacks on restricted system such as JavaScript, although, multiple execution of the "magnifier gadget" in this paper makes it detectable in hardware.  MicroScope \cite{Microscope} addresses the issue of noisy side-channels, which mandates multiple measurements for getting reliable data by utilizing core microarchitectural features to execute dynamic instruction more than once. However, this attack is detectable in hardware, as shown in \cite{EVAX2022Micro,PerSpectron}. Recent papers have enabled performing logical operation on cache signals and amplifying them to the extent that they are visible to even coarse timers, compromising the performance of the attack because of the amplification overhead~\cite{kaplan2023optimization, purnal2023showtime, katzman2023gates}. 
% % %\SMA{ , What are the weaknesses in these papers, check leakage rate, accuracy complexity requirement?Why Loki matters when these magnifiers exists}

% % \textbf{{Side-channel attacks that leak ML parameters.}}
% % Wei et al. \cite{wei2018know} were able to reconstruct the user inputs only by knowing the structure of the underlying CNN through measuring the power profile. Similarly, \cite{zhang2021stealing, tian2021remote} extracted neural network structure from FPGA using power side-channels.
% % \cite{dubey2020maskednet}, uses differential power analysis to extract parameters of a NN.

% %.\SMA{This should go to the defence recommendation. move it.}

% %\subsection{Systematic Studies of Side-Channel Attacks}
% % \para{Pandora's Box} Pandora's Box \cite{vicarte2021opening} introduced a new way of studying side channels via MLDs (Microarchitectural Leakage Descriptors) which concisely describe every possible microarchitectural state that can be left via a sequence of instructions. 

% % \para{Kaveh's prefetching study}

% % \{Didn't Daniel Gruss have a systematic study paper as well?}
% % to , not sure 





% % \subsection{Side-channel Defenses}

% % \subsubsection{Restricting fine grain timers.}
% % Cite works refer to Hacky Racers.


% % \SMA{Try not to list stuff in the background and related works like an encyclopedia.}
% %A better way to do that is to leverage the space for your purpose. What is your purpose? To present evidence supporting your scientific claim.  Think of the methods of defenses such as categorization in A Systematic Evaluation of Transient Execution Attacks and Defenses.}

% % \para{Invisispec}
% % Invisispec \cite{yan2018invisispec} attempted to mitigate cache-based covert channels by putting speculative reads into a separate microarchitectural buffer. 

% % %\para{SafeSpec}

% % %\para{DAWG}
% % DAWG \cite{kiriansky2018dawg} (Dynamically Allocated Way Guard) is a method of securely partitioning a section of the shared LLC so that an arbitrary program and a secure program can not share a cache state, mitigating cache-based covert channels.

% %\subsubsection{Detection}

% % \notema{I don't think that table is required - just cite the results and discuss them in the paper}
% % \begin{figure}[!t]
% %     \centering
% %     \includegraphics[width=\linewidth]{Figures/onchip-acc-benefits.png}
% %     \caption{ \textbf{Sustainable Computing in Risk:} Elavated workload performance, power efficiency and sustainability and more than 55\% TCO improvement with built in accelerator. Mitigating Intel AMX vulnerabilities may require hardware redesign of features that enabled these benefits. Xeon 4th Generation is named as the most sustainable data center processor.  \SMA{Create a better table TODO  please}}
% %     \label{fig:enter-label}
% % \end{figure}


% % \subsection{Built-in Accelerators: A Paradigm Shift in Computing}
% % \notema{not sure what this section is trying to tell me - looks a bit like advertising AMX...}

% % The end of Dennard scaling\notema{no idea what that means} has fueled an era of specialized accelerators, transforming the landscape of processor design.

% % In a significant paradigm shift, these accelerators are no longer solely standalone, discrete units. Instead, they are being directly integrated into CPU architectures, promising unprecedented benefits for diverse workloads while driving sustainability through efficiency.



% %\notema{is this a research question you are trying to answer? Please highlight that with a question mark or structure it in the beginning of the ection. not really sure if that is still part of the background..}
% % \subsection{Why on-chip accelerators are going to stay and simply disabling them for security will be costly----a call for urgent hardware redesign: } 

% % \textbf{The Demands of AI and Specialized Workloads:} ML models and niche applications crave customized hardware for optimal execution. On-chip accelerators deliver that tailor-made performance, often surpassing traditional CPUs and even discrete accelerators that introduce communication bottlenecks.


% % \textbf{Performance Without Bottlenecks:} 
% % Integrating accelerators within the CPU establishes high-bandwidth pathways and minimizes latency, especially crucial for fine-grained workloads. This tight coupling unlocks a new level of performance potential. %\textbf{Examples of built-in accelerators and their performance benefits}
% % For example: For AI inferencing, Intel AMX offers up to an 8.6x - 10x throughput boost~\cite{intel2023amx}. Network performance is optimized by Dynamic Load Balancer (DLB), achieving up to 96\% higher throughput while reducing latency.  
% % For data-intensive operations, Intel Data Streaming Accelerator (DSA) delivers up to 1.7x higher IOPS for SPDK-NVMe interfaces. 
% % Database operations are accelerated by up to 2.1x using RocksDB with Intel In-Memory Analytics Accelerator (IAA), streamlining analytics workflows. 
% % Finally, Intel QuickAssist Technology (QAT) significantly offloads network-related tasks, freeing up CPU cores and showcasing extraordinary efficiency gains ~\cite{colfax2023xeonscalable}.

% % \textbf{The Sustainability Advantage:} Due to their specialized nature and integrated design, on-chip accelerators are markedly more energy-efficient. This translates to lower operational costs for data centers and a reduced environmental footprint – fewer servers, less energy, and a smaller carbon impact. 


% % \textbf{The Environmental Imperative: Quantifiable CO2 Reduction} The sustainability benefits of on-chip accelerators are undeniable:
% % %\textbf{AI Inferencing:} 
% % Replacing 50 servers running 3rd Gen Intel Xeon processors with just 17 servers equipped with 4th Gen processors (featuring AMX) for AI inferencing can save a staggering 524,000 kg of CO2 emissions. %~\cite{colfax2023xeonscalable}
% % %\textbf{Media Handling:} 
% % Deploying 15 servers with 4th Gen Xeon processors (and DSA) for large media file requests can save between 206,577 kg and 611,000 kg of CO2. ~\cite{colfax2023xeonscalable}


% %\textbf{Cost.} TCO
% %Intel's 4th and 5th Generation Xeon Scalable Processors (Sapphire Rapids) exemplify the power of on-chip acceleration. 

% % {\bf Sustainable Computing in Risk:} Elavated workload performance, power efficiency and sustainability and more than 55\% TCO improvement with built in accelerator are the features that made Xeon 4th Generation to be named as the most sustainable data center processor. Mitigating Intel AMX vulnerabilities may require hardware redesign of features that enabled these benefits.  [cite]



==> contents/Old-Introduction.tex <==
we step into a new era of computing, each leap in processor technology not only boosts performance and efficiency but alters the landscape of cybersecurity threats~\cite{pandorasbox}. 
Optimizations can introduce side channels, potentially exposing sensitive data to adversaries. Simultaneously, artificial intelligence (AI) computations are increasingly becoming a significant part of the workload for various types of chips.

Matrix operations are fundamental to many AI and machine learning (ML) algorithms, especially in the training and inference processes of neural networks. Consequently, there is significant emphasis on optimizing these operations and enhancing the hardware to support them efficiently. This has led to the development and refinement of specialized processors such as GPUs, TPUs, and other AI-specific chips designed to handle these intensive computational tasks more effectively.

In a major change, AI accelerators are no longer solely standalone, discrete units. Instead, they are directly integrated into CPU architectures\cite{jeong2021rasa,jeong2023vegeta,nassif2022sapphire, elster2022nvidia}. This integration creates fast data paths and reduces delays. As a result, it boosts performance and improves energy efficiency compared to separate units.

Intel Advanced Matrix Extensions (AMX) is an on-chip accelerator designed to enhance the computational capabilities of modern processors. Integrated into Intel's latest processor architectures, specifically starting with the 4th Gen Intel Xeon Scalable processors code-named Sapphire Rapids, Intel AMX provides specialized hardware support for high-throughput operations required for matrix multiplication. By significantly boosting the efficiency and speed of these operations, Intel AMX enables faster training and inference times, leading to more responsive AI applications and more efficient use of system resources ~\cite{intel2022amx}. 



In this paper, we demonstrate that the execution times of AMX multiplication are not fixed and that AMX multiplication operates in five distinct power states, ranging from 16 to 20,000 cycles. %(Figure~\ref{fig:Power_Stages}). 
We also discovered that the execution time of AMX multiplication in high-latency power states depends on the specific values of the data it processes. This creates exploitable timing differences that can be used to infer sensitive information, such as the weights of a neural network model or the input data. We present the techniques required to practically exploit this side-channel vulnerability in neural networks. We show that it is possible to leak the 64 hidden binary weights of a neural network solely by measuring the execution time, achieving 100\% accuracy after a duration of 50 minutes.

==> contents/Related.tex <==
\section{Related Works}

%\notema{add some intro words here}

% In this section, we present a background on related micro-architectural attacks, an overview of built-in accelerators and their benefits, as well as a background on Intel AMX instruction and architecture.  


%\subsection{Microarchitectural Side-channel Attacks}
%\{Overview of side-channel attacks, defining covert channel, leakage gadget, etc?}\SMA{ to : No we don't need to explain those.There won't be space.} 
%\SMA{For each attack, add their threat model and parameters that matter to CVSS, such as scope, vector,  complexity, and information that would build context around **your paper's findings**. To help them better appreciate your findings. Not to teach a whole Wikipedia in half a page. }
%\subsubsection{Cache attacks}
%The oldest side-channel attacks are cache attacks. 
%\notema{this section requires some more polishing}
%\notema{osvik: Cache Attacks and Countermeasures: the Case of AES. should be cited as well for prime+probe}

% \begin{figure}[!t]
%     \centering
%    \includegraphics[width=\linewidth]{images/AMXarch_new_v1.pdf} 
%     \caption{Intel AMX Architecture Overview}
%     \label{fig:AMX-arch}
% \end{figure}

% \textbf{{Intel AMX Architecture and Instructions.}}
% Intel AMX is an integrated accelerator introduced with the 4th Gen Intel Xeon Scalable processors, specifically engineered to boost the efficiency of matrix computations that are essential for artificial intelligence and high-performance computing applications. Figure~\ref{fig:AMX-arch} illustrates the Intel AMX architecture.

% AMX introduces a new set of registers and instructions. The registers in Intel AMX are known as Tiles, a new concept in Intel CPUs that provide a matrix of data registers, as opposed to the traditional vector registers seen in previous SIMD architectures like AVX-512. AMX includes 8 Tile registers, each capable of holding up to 16 rows with 64 bytes per row, amounting to a total of 1 KB per Tile. The number of rows and the number of bytes per row can be adjusted using the LDTILECFG instruction, and this configuration information is stored as metadata in a control register known as TILECFG. Once this configuration is set, AMX instructions such as load, store, and matrix multiplication will operate according to the specified dimensions for each Tile. Intel AMX instructions are synchronized with the Intel Architecture host (IA host) instruction stream, and the Tile loads and stores are coherent with the host memory \cite{Intel_Arc_Ins_Set_Extensions}.

% Tile Matrix Multiply unit (TMUL) serves as the accelerator engine for executing multiplication calculations. When using full-size Tile operands, the latency of the multiplication instruction is 52 cycles, while pipelining allows for a throughput of 16 cycles. Intel AMX supports two data types: BF16 and INT8. Consequently, it can perform 512 multiplications and 512 additions per cycle for BF16 and 1024 multiplications and 1024 additions per cycle for INT8 \cite{IntelOptRefManual}. 

% AMX instructions utilize port 5 as their dedicated execution port. When two hyper-threads are active within a core, they compete for the same resources to execute AMX instructions.


\paragrabf{Cache attacks.}
Cache attacks exploit timing differences caused by loading data from different cache levels or the DRAM.
In \PrimeProbe~\cite{prime_probe,osvik2006cache}, the attacker "primes" a cache set and waits for the victim to execute, tracking evictions. Flush+Reload \cite{flush+reload} flushes a cache line and checks if it was filled by the victim.
% Flush+Reload \cite{flush+reload} 
% uses the presence or absence of a variable shared between the attacker and victim (e.g. in a shared library) to deduce a victim's program path.
Flush+Flush attack ~\cite{GrussFlushFlush} relies on the execution time variation of the flush instruction.

%\subsubsection{Speculative \& Transient Attacks} 

\paragrabf{Transient-execution attacks.}
% Spectre \cite{kocher2020spectre}
%is a class of attacks that abuse mechanisms that result in jumps in code (e.g. branch predictor, pattern history table) to speculatively execute certain instructions that have a measurable effect on the microarchitecture (but not the architecture). For example, in Spectre-v1
% %\notema{Use the classification of Canella et al} 
% the branch predictor is mistrained on a particular branch with a value that points to an in-bound variable. The attacker then changes the value to point to an out-of-bounds and causes the branch to execute. Due to out-of-order execution, for a small amount of cycles the incorrect code can execute which, when the measurable microarchitectural change caused by the code is dependent on the out-of-bounds value, can lead to an attacker being able to read the entirety of a process's address space. Other attacks include 
% and Meltdown 
% \cite{meltdown};
Spectre \cite{kocher2020spectre} exploits speculative execution of an operation that would not occur during correct execution path of the program. Meltdown-type attacks \cite{meltdown} exploit delayed
exception handling during out-of-order execution.
% e.g. there was a null pointer access but the check for the exception was executed after other transient instructions were being executed.
Forshadow~\cite{van2018foreshadow}
%\notema{what about foreshadow?} 
exploits a bug in Intel CPUs that led to imperfect isolation of the SGX enclave context, Load Value Injection \cite{lvi} induces execution based on malicious values injected in various microarchitectural buffers, Fallout \cite{canella2019fallout} leaks the contents of the store buffer, and RIDL \cite{ridl} and Zombieload \cite{schwarz2019zombieload} leak the contents of the line fill buffer.


\paragrabf{Software-based power side-channel attacks.}
%\subsubsection{Software Power Side channel attacks like Platypus}
Platypus \cite{Lipp2021Platypus} exploits the RAPL (Running Average Power Limit) driver, to infer the internal state of a program, even inside an SGX enclave. This vulnerability was mitigated by kernel updates restricting RAPL access and Intel microcode updates changing how power is reported in the context of SGX.
%for everything except SGX 
% by restricting RAPL access to privileged users using a kernel update and was mitigated for privileged users through an Intel microcode update that decorrelated the power report from operands in the context of an SGX enclave. 
%\{This is wrong. Intel released a microcode update that changes how power is reported when in the context of an SGX enclave}. \SMA{Who wrote that? Martin?  it seems like someone wrote that was confident. Ohhh I see this is right because with malicious OS, OS has access to RAPL? But Micro code fixed it. So don't say that if we are not sure. }
Collide+Power~\cite{kogler2023collide+} uses a differential power measurement technique involving pairs of inputs with their inverses to leak victim data coexisting with attacker data in the same microarchitectural buffers. 
%\subsubsection{Attacks that exploit accelerators}
% Grand Pwning Unit \cite{frigo2018grand} explored using GPUs to accelerate microarchitectural attacks, specifically RowHammer\notema{Not sure if Rowhammer and GPUs are relevant here..}. They found that since the GPU is accessible from Javascript, it is possible to mount a Rowhammer attack by injecting Javascript code into a web browser. 



%\subsubsection{Remote attacks}
% \paragrabf{Remote timing attacks.}
% Many remote side-channel attacks were solely focusing on cryptographic primitives such as AES or RSA ~\cite{Aciicmez2007d,Brumley2003Remote,Bernstein2005,Zhao2009cache,Jayasinghe2010remote,Aly2013attacking,Saraswat2014}.
% Irazoqui \etal\cite{Irazoqui2015Lucky} attacked TLS in a remote setup leveraging cache timing differences.
% Schwarz \etal\cite{schwarz2019netspectre} demonstrated Spectre attacks in a fully remote setup (with controlled network traffic) leveraging both a cache side channel and an AVX side channel to remotely exfiltrate data.
% \cite{VanGoethem2020Timeless} makes use of the relative timing difference in response time to tackle existing jitter in networks. 
% Moreover, remote attacks were created leaking data by exploiting operating system optimizations ~\cite{Gruss2019page,Schwarzl2022Remote}, DVFS to attack post-quantum cryptography~\cite{wang2022hertzbleed} and the compression ratio~\cite{schwarzl2023practical}.
% %Memory compression attacks work only on programs that employ memory compression like web servers; Loki is more general than this functioning on any program that listens for network requests and utilizes the AMX unit. Hertzbleed relies on dynamic voltage and frequency (DVFS) scaling while Loki works independently of DVFS.

% %\SMA{The immediate  question comes in mind is why we didn't compare with all of these? Are they out of scope? Are they about something else? What is common what is not common. This section without a conclusion in comparison with our work kills our paper. Our paper gets killed without having it as well. Justify. TODO . Also after reading it it feels like our work is not novel so for example say, "Although these works studied remote attacks in this and that condition but they didn't study this or couldnt do that or their impact was weak... on the other hand we .... the comparison with Netspectre and blah blah is given in section blah"}

% \noindent\textbf{{Signal Amplification.}}
% Amplifying a side channel's signal strength, e.g. the timing difference, can significantly reduce noise.
% Roettger and Janc~\cite{Roettger2021A} leveraged the PLRU cache replacement policy in the L1 to arbitrarily amplify a single cache hit. However, it relies on the cache and thus any cache side-channel defense, e.g.\ \cite{Invisispec}, would mitigate this issue. Additionally, this method may be detectable in hardware.
% Hacky Racers~\cite{HackyRacers2023ASPLOS} %introduced "racing gadgets" and "magnifier gadgets" by exploiting 
% exploited instruction-level parallelism enabling timing attacks on restricted system such as JavaScript, although, multiple execution of the "magnifier gadget" in this paper makes it detectable in hardware.  MicroScope \cite{Microscope} addresses the issue of noisy side-channels, which mandates multiple measurements for getting reliable data by utilizing core microarchitectural features to execute dynamic instruction more than once. However, this attack is detectable in hardware, as shown in \cite{EVAX2022Micro,PerSpectron}. Recent papers have enabled performing logical operation on cache signals and amplifying them to the extent that they are visible to even coarse timers, compromising the performance of the attack because of the amplification overhead~\cite{kaplan2023optimization, purnal2023showtime, katzman2023gates}. 
% %\SMA{ , What are the weaknesses in these papers, check leakage rate, accuracy complexity requirement?Why Loki matters when these magnifiers exists}

\textbf{{Side-channel attacks that leak ML parameters.}}
Wei et al. \cite{wei2018know} were able to reconstruct the user inputs only by knowing the structure of the underlying CNN through measuring the power profile. Similarly, \cite{zhang2021stealing, tian2021remote} extracted neural network structure from FPGA using power side-channels.
\cite{dubey2020maskednet}, uses differential power analysis to extract parameters of a NN.

% {This paragraph needs review. (Not well written.)}

% \SMA{I agree,  it shouldn't be only about what it leaks (Impact) for example Forshadow leaks kernel, it should be about their method Key idea/root cause of vulnerability and also Impact.}
% \notema{canella defined a difference between spectre and meltdown - spectre exploits mispredictions by the branch predictor leading to transient accesses while for meltdown-type effects the underlying root cause is delayed
% exception handling during out-of-order execution. e.g. there was a null pointer access but the check for the exception was executed after other transient instructions were being executed.}

% %\subsubsection{Rowhammer}
% \paragrabf{Software-based power side-channel attacks.}
% %\subsubsection{Software Power Side channel attacks like Platypus}
% Platypus \cite{Lipp2021Platypus} exploits the RAPL (Running Average Power Limit) driver, to infer the internal state of a program, even inside an SGX enclave. This vulnerability was mitigated by kernel updates restricting RAPL access and Intel microcode updates changing how power is reported in the context of SGX.
% %for everything except SGX 
% % by restricting RAPL access to privileged users using a kernel update and was mitigated for privileged users through an Intel microcode update that decorrelated the power report from operands in the context of an SGX enclave. 
% %\{This is wrong. Intel released a microcode update that changes how power is reported when in the context of an SGX enclave}. \SMA{Who wrote that? Martin?  it seems like someone wrote that was confident. Ohhh I see this is right because with malicious OS, OS has access to RAPL? But Micro code fixed it. So don't say that if we are not sure. }
% Collide+Power~\cite{kogler2023collide+} uses a differential power measurement technique involving pairs of inputs with their inverses to leak victim data coexisting with attacker data in the same microarchitectural buffers. 
% %\subsubsection{Attacks that exploit accelerators}
% % Grand Pwning Unit \cite{frigo2018grand} explored using GPUs to accelerate microarchitectural attacks, specifically RowHammer\notema{Not sure if Rowhammer and GPUs are relevant here..}. They found that since the GPU is accessible from Javascript, it is possible to mount a Rowhammer attack by injecting Javascript code into a web browser. 



% %\subsubsection{Remote attacks}
% \paragrabf{Remote timing attacks.}
% Many remote side-channel attacks were solely focusing on cryptographic primitives such as AES or RSA ~\cite{Aciicmez2007d,Brumley2003Remote,Bernstein2005,Zhao2009cache,Jayasinghe2010remote,Aly2013attacking,Saraswat2014}.
% Irazoqui \etal\cite{Irazoqui2015Lucky} attacked TLS in a remote setup leveraging cache timing differences.
% Schwarz \etal\cite{schwarz2019netspectre} demonstrated Spectre attacks in a fully remote setup (with controlled network traffic) leveraging both a cache side channel and an AVX side channel to remotely exfiltrate data.
% \cite{VanGoethem2020Timeless} makes use of the relative timing difference in response time to tackle existing jitter in networks. 
% Moreover, remote attacks were created leaking data by exploiting operating system optimizations ~\cite{Gruss2019page,Schwarzl2022Remote}, DVFS to attack post-quantum cryptography~\cite{wang2022hertzbleed} and the compression ratio~\cite{schwarzl2023practical}.
% %Memory compression attacks work only on programs that employ memory compression like web servers; Loki is more general than this functioning on any program that listens for network requests and utilizes the AMX unit. Hertzbleed relies on dynamic voltage and frequency (DVFS) scaling while Loki works independently of DVFS.

% %\SMA{The immediate  question comes in mind is why we didn't compare with all of these? Are they out of scope? Are they about something else? What is common what is not common. This section without a conclusion in comparison with our work kills our paper. Our paper gets killed without having it as well. Justify. TODO . Also after reading it it feels like our work is not novel so for example say, "Although these works studied remote attacks in this and that condition but they didn't study this or couldnt do that or their impact was weak... on the other hand we .... the comparison with Netspectre and blah blah is given in section blah"}

% \textbf{{Signal Amplification.}}
% Amplifying a side channel's signal strength, e.g. the timing difference, can significantly reduce noise.
% Roettger and Janc~\cite{Roettger2021A} leveraged the PLRU cache replacement policy in the L1 to arbitrarily amplify a single cache hit. However, it relies on the cache and thus any cache side-channel defense, e.g.\ \cite{Invisispec}, would mitigate this issue. Additionally, this method may be detectable in hardware.
% Hacky Racers~\cite{HackyRacers2023ASPLOS} %introduced "racing gadgets" and "magnifier gadgets" by exploiting 
% exploited instruction-level parallelism enabling timing attacks on restricted system such as JavaScript, although, multiple execution of the "magnifier gadget" in this paper makes it detectable in hardware.  MicroScope \cite{Microscope} addresses the issue of noisy side-channels, which mandates multiple measurements for getting reliable data by utilizing core microarchitectural features to execute dynamic instruction more than once. However, this attack is detectable in hardware, as shown in \cite{EVAX2022Micro,PerSpectron}. Recent papers have enabled performing logical operation on cache signals and amplifying them to the extent that they are visible to even coarse timers, compromising the performance of the attack because of the amplification overhead~\cite{kaplan2023optimization, purnal2023showtime, katzman2023gates}. 
% %\SMA{ , What are the weaknesses in these papers, check leakage rate, accuracy complexity requirement?Why Loki matters when these magnifiers exists}

% \textbf{{Side-channel attacks that leak ML parameters.}}
% Wei et al. \cite{wei2018know} were able to reconstruct the user inputs only by knowing the structure of the underlying CNN through measuring the power profile. Similarly, \cite{zhang2021stealing, tian2021remote} extracted neural network structure from FPGA using power side-channels.
% \cite{dubey2020maskednet}, uses differential power analysis to extract parameters of a NN.

%.\SMA{This should go to the defence recommendation. move it.}

%\subsection{Systematic Studies of Side-Channel Attacks}
% \para{Pandora's Box} Pandora's Box \cite{vicarte2021opening} introduced a new way of studying side channels via MLDs (Microarchitectural Leakage Descriptors) which concisely describe every possible microarchitectural state that can be left via a sequence of instructions. 

% \para{Kaveh's prefetching study}

% \{Didn't Daniel Gruss have a systematic study paper as well?}
% to , not sure 





% \subsection{Side-channel Defenses}

% \subsubsection{Restricting fine grain timers.}
% Cite works refer to Hacky Racers.


% \SMA{Try not to list stuff in the background and related works like an encyclopedia.}
%A better way to do that is to leverage the space for your purpose. What is your purpose? To present evidence supporting your scientific claim.  Think of the methods of defenses such as categorization in A Systematic Evaluation of Transient Execution Attacks and Defenses.}

% \para{Invisispec}
% Invisispec \cite{yan2018invisispec} attempted to mitigate cache-based covert channels by putting speculative reads into a separate microarchitectural buffer. 

% %\para{SafeSpec}

% %\para{DAWG}
% DAWG \cite{kiriansky2018dawg} (Dynamically Allocated Way Guard) is a method of securely partitioning a section of the shared LLC so that an arbitrary program and a secure program can not share a cache state, mitigating cache-based covert channels.

%\subsubsection{Detection}

% \notema{I don't think that table is required - just cite the results and discuss them in the paper}
% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=\linewidth]{Figures/onchip-acc-benefits.png}
%     \caption{ \textbf{Sustainable Computing in Risk:} Elavated workload performance, power efficiency and sustainability and more than 55\% TCO improvement with built in accelerator. Mitigating Intel AMX vulnerabilities may require hardware redesign of features that enabled these benefits. Xeon 4th Generation is named as the most sustainable data center processor.  \SMA{Create a better table TODO  please}}
%     \label{fig:enter-label}
% \end{figure}


% \subsection{Built-in Accelerators: A Paradigm Shift in Computing}
% \notema{not sure what this section is trying to tell me - looks a bit like advertising AMX...}

% The end of Dennard scaling\notema{no idea what that means} has fueled an era of specialized accelerators, transforming the landscape of processor design.

% In a significant paradigm shift, these accelerators are no longer solely standalone, discrete units. Instead, they are being directly integrated into CPU architectures, promising unprecedented benefits for diverse workloads while driving sustainability through efficiency.



%\notema{is this a research question you are trying to answer? Please highlight that with a question mark or structure it in the beginning of the ection. not really sure if that is still part of the background..}
% \subsection{Why on-chip accelerators are going to stay and simply disabling them for security will be costly----a call for urgent hardware redesign: } 

% \textbf{The Demands of AI and Specialized Workloads:} ML models and niche applications crave customized hardware for optimal execution. On-chip accelerators deliver that tailor-made performance, often surpassing traditional CPUs and even discrete accelerators that introduce communication bottlenecks.


% \textbf{Performance Without Bottlenecks:} 
% Integrating accelerators within the CPU establishes high-bandwidth pathways and minimizes latency, especially crucial for fine-grained workloads. This tight coupling unlocks a new level of performance potential. %\textbf{Examples of built-in accelerators and their performance benefits}
% For example: For AI inferencing, Intel AMX offers up to an 8.6x - 10x throughput boost~\cite{intel2023amx}. Network performance is optimized by Dynamic Load Balancer (DLB), achieving up to 96\% higher throughput while reducing latency.  
% For data-intensive operations, Intel Data Streaming Accelerator (DSA) delivers up to 1.7x higher IOPS for SPDK-NVMe interfaces. 
% Database operations are accelerated by up to 2.1x using RocksDB with Intel In-Memory Analytics Accelerator (IAA), streamlining analytics workflows. 
% Finally, Intel QuickAssist Technology (QAT) significantly offloads network-related tasks, freeing up CPU cores and showcasing extraordinary efficiency gains ~\cite{colfax2023xeonscalable}.

% \textbf{The Sustainability Advantage:} Due to their specialized nature and integrated design, on-chip accelerators are markedly more energy-efficient. This translates to lower operational costs for data centers and a reduced environmental footprint – fewer servers, less energy, and a smaller carbon impact. 


% \textbf{The Environmental Imperative: Quantifiable CO2 Reduction} The sustainability benefits of on-chip accelerators are undeniable:
% %\textbf{AI Inferencing:} 
% Replacing 50 servers running 3rd Gen Intel Xeon processors with just 17 servers equipped with 4th Gen processors (featuring AMX) for AI inferencing can save a staggering 524,000 kg of CO2 emissions. %~\cite{colfax2023xeonscalable}
% %\textbf{Media Handling:} 
% Deploying 15 servers with 4th Gen Xeon processors (and DSA) for large media file requests can save between 206,577 kg and 611,000 kg of CO2. ~\cite{colfax2023xeonscalable}


%\textbf{Cost.} TCO
%Intel's 4th and 5th Generation Xeon Scalable Processors (Sapphire Rapids) exemplify the power of on-chip acceleration. 

% {\bf Sustainable Computing in Risk:} Elavated workload performance, power efficiency and sustainability and more than 55\% TCO improvement with built in accelerator are the features that made Xeon 4th Generation to be named as the most sustainable data center processor. Mitigating Intel AMX vulnerabilities may require hardware redesign of features that enabled these benefits.  [cite]




\paragrabf{Hertzbleed \cite{wang2022hertzbleed}.}
Hertzbleed leverages dynamic voltage and frequency scaling (DVFS) to transform power side-channel attacks into timing attacks. By exploiting the timing differences caused by frequency variations, even remote attacks become feasible. For instance, in an attack against Supersingular Isogeny Key Encapsulation (SIKE), they managed to recover 378 bits of the private key within 36 hours. Although this attack shares similarities with our work in exploiting frequency changes, DVFS can be managed by the CPU core and disabled in BIOS settings to mitigate the Hertzbleed attack. However, in our case, disabling DVFS is not a viable countermeasure since AMX, an on-chip accelerator, manages its power and frequency independently.

\paragrabf{Collide+Power \cite{kogler2023collide+}.}
The Collide+Power research focuses on the power leakage of the memory hierarchy via Running Average Power Limit (RAPL). If RAPL is unavailable, monitoring can be done through a throttling side-channel, albeit requiring more measurements. They demonstrated two types of attacks: Meltdown-style and Microarchitectural Data Sampling (MDS)-style. In Meltdown-style, targeting a shared cache among two processes on different cores, theoretically, one bit can be leaked in 99.95 days with power limit control or 2.86 years with stress-induced throttling. In MDS-style, where both victim and attacker run on different logical cores of the same physical core, data can be leaked from the L1/L2 cache at a rate of 4.82 bits per hour. Disabling simultaneous multithreading can mitigate MDS-style attacks. Generally, RAPL being a privileged interface is not accessible to unprivileged attackers, and throttling can be disabled by turning off DVFS.

\paragrabf{Platypus \cite{Lipp2021Platypus}.}
The Platypus attack reconstructed 509 RSA key bits using RAPL MSRs within Intel SGX enclaves. However, this attack vector has been mitigated by making RAPL a privileged interface.

\paragrabf{Neural Network Specific Attacks.}
Several studies have attacked neural network accelerators using power side channels. In the work by Wei et al. \cite{wei2018know}, an FPGA-based convolutional neural network accelerator was attacked, requiring physical access to recover the model's input image with up to 89\% accuracy. Effective mitigations include masking and random scheduling, although masking introduces significant overheads, as demonstrated in MaskedNet \cite{dubey2020maskednet}, increasing latency and area costs by 2.8x and 2.3x, respectively.

Open DNN Box \cite{Xiang2019OpenDB} inferred the weight sparsity of neural network models with 96.5\% accuracy on average. CSI NN \cite{236204} used power and electromagnetic traces to infer information about weights and architecture in fully connected neural networks. DeepEM \cite{Yu2020DeepEMDN} and DeepSniffer \cite{Hu2020DeepSnifferAD} collected electromagnetic traces to glean architectural information, with DeepEM specifically targeting binarized neural networks. Cache Telepathy \cite{244042}, GANRED \cite{Liu2020GANREDGR}, and DeepRecon \cite{Hong2018SecurityAO} employed well-known cache side channels like Flush+Reload and Prime+Probe to gather neural network insights. For these cache attacks, the attacker runs locally, and the presence of a shared cache is necessary. In contrast, our Thor attack doesn't need physical access or shared cache. It introduces a novel, data-dependent timing side-channel vulnerability specific to Intel AMX accelerators.

In the work by Gongye et al. \cite{9218707}, they attacked DNNs using a floating-point timing side channel to obtain weights and biases. They took advantage of the drastically different execution times for floating-point multiplication and addition in certain scenarios, such as when dealing with subnormal values, to launch their attack. However, with modern accelerators like Intel AMX, this floating-point timing vulnerability has been eliminated. Now, the execution time for tile multiplication remains constant, even for special cases like zero inputs. Specifically, the latency is fixed at 52 cycles and the throughput is 16. Despite this, to attack DNNs with more than one layer, cache monitoring or physical access is still required to measure the execution time of each layer.

==> contents/RelatedWorks.tex <==
Here, we discuss significant related works and potential countermeasures relevant to our Thor attack.

\paragrabf{Hertzbleed \cite{wang2022hertzbleed}.}
Hertzbleed leverages dynamic voltage and frequency scaling (DVFS) to transform power side-channel attacks into timing attacks. By exploiting the timing differences caused by frequency variations, even remote attacks become feasible. For instance, in an attack against Supersingular Isogeny Key Encapsulation (SIKE), they managed to recover 378 bits of the private key within 36 hours. Although this attack shares similarities with our work in exploiting frequency changes, DVFS can be managed by the CPU core and disabled in BIOS settings to mitigate the Hertzbleed attack. However, in our case, disabling DVFS is not a viable countermeasure since AMX, an on-chip accelerator, manages its power and frequency independently.

\paragrabf{Collide+Power \cite{kogler2023collide+}.}
The Collide+Power research focuses on the power leakage of the memory hierarchy via Running Average Power Limit (RAPL). If RAPL is unavailable, monitoring can be done through a throttling side-channel, albeit requiring more measurements. They demonstrated two types of attacks: Meltdown-style and Microarchitectural Data Sampling (MDS)-style. In Meltdown-style, targeting a shared cache among two processes on different cores, theoretically, one bit can be leaked in 99.95 days with power limit control or 2.86 years with stress-induced throttling. In MDS-style, where both victim and attacker run on different logical cores of the same physical core, data can be leaked from the L1/L2 cache at a rate of 4.82 bits per hour. Disabling simultaneous multithreading can mitigate MDS-style attacks. Generally, RAPL being a privileged interface is not accessible to unprivileged attackers, and throttling can be disabled by turning off DVFS.

\paragrabf{Platypus \cite{Lipp2021Platypus}.}
The Platypus attack reconstructed 509 RSA key bits using RAPL MSRs within Intel SGX enclaves. However, this attack vector has been mitigated by making RAPL a privileged interface.

\paragrabf{Neural Network Specific Attacks.}
Several studies have attacked neural network accelerators using power side channels. In the work by Wei et al. \cite{wei2018know}, an FPGA-based convolutional neural network accelerator was attacked, requiring physical access to recover the model's input image with up to 89\% accuracy. Effective mitigations include masking and random scheduling, although masking introduces significant overheads, as demonstrated in MaskedNet \cite{dubey2020maskednet}, increasing latency and area costs by 2.8x and 2.3x, respectively.

Open DNN Box \cite{Xiang2019OpenDB} inferred the weight sparsity of neural network models with 96.5\% accuracy on average. CSI NN \cite{236204} used power and electromagnetic traces to infer information about weights and architecture in fully connected neural networks. DeepEM \cite{Yu2020DeepEMDN} and DeepSniffer \cite{Hu2020DeepSnifferAD} collected electromagnetic traces to glean architectural information, with DeepEM specifically targeting binarized neural networks. Cache Telepathy \cite{244042}, GANRED \cite{Liu2020GANREDGR}, and DeepRecon \cite{Hong2018SecurityAO} employed well-known cache side channels like Flush+Reload and Prime+Probe to gather neural network insights. For these cache attacks, the attacker runs locally, and the presence of a shared cache is necessary. In contrast, our Thor attack doesn't need physical access or shared cache. It introduces a novel, data-dependent timing side-channel vulnerability specific to Intel AMX accelerators.

In the work by Gongye et al. \cite{9218707}, they attacked DNNs using a floating-point timing side channel to obtain weights and biases. They took advantage of the drastically different execution times for floating-point multiplication and addition in certain scenarios, such as when dealing with subnormal values, to launch their attack. However, with modern accelerators like Intel AMX, this floating-point timing vulnerability has been eliminated. Now, the execution time for tile multiplication remains constant, even for special cases like zero inputs. Specifically, the latency is fixed at 52 cycles and the throughput is 16. Despite this, to attack DNNs with more than one layer, cache monitoring or physical access is still required to measure the execution time of each layer.

% \paragrabf{Potential Countermeasures.}
% Eliminating the cooldown state could defend against Thor but at a high power cost since Intel AMX is an energy-intensive accelerator designed for AI tasks. Keeping AMX continuously active would be power-prohibitive.

% Masking is a proven countermeasure for protecting AI model parameters against power side-channel attacks and could be adapted for future AMX versions despite the performance overhead. Additionally, machine learning models should incorporate techniques to detect unusual usage patterns, which can help identify and thwart attacks attempting to infer parameter values using methods similar to our AMX-type attack. One well-known countermeasure to these timing attacks is to coarsen the timer. By reducing the timer's precision, it becomes much harder for attackers to measure the subtle differences in execution times that they rely on for their exploits.

% In summary, while various countermeasures exist for different attack vectors, protecting against Thor on Intel AMX accelerators requires novel approaches to power and frequency management alongside traditional techniques.




==> contents/SecAnalysis.tex <==

\section{Security Analysis}

\subsection{Success Rate Analysis}
After extensive experiments, the configurable parameters in Algorithm \ref{alg:alg1} were selected to the following values: \(N=10000\), \(M=40\), \(L=20\), \(K=3\), \(\alpha=0.9\), and \(\gamma=1.13\), which were effective in demonstrating the outcome. Prolonging the attack duration reduces noise in the scores and enhances the success rate of accurately determining the weights. 

%\begin{figure}[!htbp]
%\centerline{\includegraphics[width=0.4\textwidth]%{images/ML_Attack_Successful_Rate_v3.pdf}}
%\caption{Impact of Attack Duration on the Success Rate of Weight Determination.  if you leak for example 100 different perceptrons successfully you can plot that as well. If you remember a reviewer was asking whether you can leak a particular set of weights or all  combination. {\color{red}maybe show this with bar chart? } }
%\label{fig:ML_SuccessRate}
%\end{figure}

\begin{figure}[h!]
\centering
\begin{tikzpicture}
    \begin{axis}[
        xlabel={Attack Duration (minute)},
        ylabel={Successful Rate},
        legend pos=outer north east,
        font=\scriptsize,
        xlabel style={yshift=5pt},
        ylabel style={yshift=-15pt},
        width=\linewidth*1,
        height=\linewidth*0.6,
        xmax=100, xmin=0,
        legend style={
                legend columns=-1,
                at={(0.5,1.16)},
                anchor=north, 
                font=\tiny,
                /tikz/column 2/.style={column sep=5pt}, 
            },
    ]
    \addplot[
        line width=2pt,
        color=darkgray,
    ] table {Diagrams/Data/accuracy.txt};

    \end{axis}
\end{tikzpicture}
\caption{Impact of Attack Duration on the Success Rate of Weight Determination.  if you leak for example 100 different perceptrons successfully you can plot that as well. If you remember a reviewer was asking whether you can leak a particular set of weights or all  combination.}
\label{fig:ML_SuccessRate}
\end{figure}

Figure \ref{fig:ML_SuccessRate} shows success rates increasing with longer attack durations, from 60\% at 5 minutes to a complete 100\% success rate at 50 minutes (0.02 bit/s) and beyond. Since cooling down the AMX is necessary for every timing measurement, over 99\% of the attack duration is consumed by cooling delays. Additionally, the results of the algorithm for two different attack durations are shown in Figure \ref{fig:LeakedWeights}. 

\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{thor_black_white_compare.png}
    \caption{{\color{red} Add the conclusion of this figure.  TODO improve the fonts and readability of the figure. }}
    \label{fig:thorleakage}
\end{figure}

{\color{red} , You can add the success rate plot here and compare. I pasted the copy you sent me. Please improve it.}


%\begin{figure}
%    \centering
%    \includegraphics[width=0.6\linewidth]{thor_black_white_compare.png}
%    \caption{{\color{red} Add the conclusion of this figure.  TODO improve the fonts and readability of the figure. }}
%    \label{fig:enter-label}
%\end{figure}
%\begin{figure}[!htbp]
%\centerline{\includegraphics[width=.8\linewidth]{images/Example.pdf}}
%\caption{{\color{red} Use two symbols like circles and stars or rectangular, that can be distinguishable in gray scale if you print with black and white. }Output of the side-channel attack for two different attack durations. In both figures, green markers represent weights of 0, and orange markers represent weights of 1. }
%\label{fig:LeakedWeights}
%\end{figure}


\begin{figure}[h!]
    \centering
    \begin{minipage}{0.5\linewidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                xlabel={Weight Index},
                ylabel={Score1/Score0},
                legend pos=outer north east,
                xmin=-1, xmax=65,
                font=\scriptsize,
                xlabel style={yshift=5pt},
                ylabel style={yshift=-15pt},
                width=1.1\linewidth,
                height=\linewidth,
            ]
                \addplot[
                    thick,
                    only marks,
                    line width=1.5pt,
                    mark=o,
                    mark size=1,
                    color=darkgray,
                    forget plot
                ] table {Diagrams/Data/30_min_0.txt};

                \addplot[
                    thick,
                    only marks,
                    mark=triangle,
                    line width=1.5pt,
                    mark size=1,
                    color=darkgray,
                    forget plot
                ] table {Diagrams/Data/30_min_1.txt};

                \addplot[
                    thick,
                    domain=0:70,
                    samples=2, 
                    color=black,
                    dashed,
                    forget plot
                ] {1.13};
            \end{axis}
            \node[black, thick] at (1.2,3.2) {\small (a) Attack Duration: 75 minutes};
        \end{tikzpicture}
    \end{minipage}\hfill
    \begin{minipage}{0.5\linewidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                xlabel={Weight Index},
                ylabel={Score1/Score0},
                legend pos=outer north east,
                xmin=-1, xmax=65,
                font=\scriptsize,
                xlabel style={yshift=5pt},
                ylabel style={yshift=-15pt},
                width=1.1\linewidth,
                height=\linewidth,
            ]
                \addplot[
                    thick,
                    only marks,
                    line width=1.5pt,
                    mark=o,
                    mark size=1,
                    color=darkgray,
                    forget plot
                ] table {Diagrams/Data/75_min_0.txt};

                \addplot[
                    thick,
                    only marks,
                    mark=triangle,
                    line width=1.5pt,
                    mark size=1,
                    color=darkgray,
                    forget plot
                ] table {Diagrams/Data/75_min_1.txt};

                \addplot[
                    thick,
                    domain=0:70,
                    samples=2, 
                    color=black,
                    dashed,
                    forget plot
                ] {1.13};
            \end{axis}
            \node[black, thick] at (1.4,3.2) {\small (b) Attack Duration: 30 minutes};
        \end{tikzpicture}
    \end{minipage}
    \caption{Output of the side-channel attack for two different attack durations. In both figures, green markers represent weights of 0, and orange markers represent weights of 1.}
    \label{fig:LeakedWeights}
\end{figure}


\subsection{Attack Requirements Analysis}
\subsubsection{Frequency Scaling Analysis}
{\color{red} add your frequency and clock analysis results and explanation here, explain in depth. }



% \paragrabf{Potential Countermeasures.}
% Eliminating the cooldown state could defend against Thor but at a high power cost since Intel AMX is an energy-intensive accelerator designed for AI tasks. Keeping AMX continuously active would be power-prohibitive.

% Masking is a proven countermeasure for protecting AI model parameters against power side-channel attacks and could be adapted for future AMX versions despite the performance overhead. Additionally, machine learning models should incorporate techniques to detect unusual usage patterns, which can help identify and thwart attacks attempting to infer parameter values using methods similar to our AMX-type attack. One well-known countermeasure to these timing attacks is to coarsen the timer. By reducing the timer's precision, it becomes much harder for attackers to measure the subtle differences in execution times that they rely on for their exploits.

% In summary, while various countermeasures exist for different attack vectors, protecting against Thor on Intel AMX accelerators requires novel approaches to power and frequency management alongside traditional techniques.



% \input{contents/RelatedWorks}


\subsection{NN leaked Parameters Comparison}
{\color{red} , compare other NN attacks and what they leaked here vs. what can be leaked by Thor.}



==> contents/acknowledgments.tex <==
This should be a simple paragraph before the References to thank those individuals and institutions who have supported your work on this article.

==> contents/attack.tex <==
\label{sec:ML_Network}
We present a proof of concept for a side-channel attack that leaks the zero weights of the first layer of a neural network by measuring execution time. The techniques we propose for this attack can be applied to similar models implemented with Intel AMX. 

This attack exploits timing differences observed when TMUL enters the Warm State, specifically taking advantage of variations in execution times that occur due to the presence of zeros in the operands. Note that our attack does not require any additional information about the memory layout.


\paragrabf{Setup.}
Our experimental setup involves a single-layer neural network constructed with 64 weights. Each weight is dedicated to one input element and the network is implemented using Intel AMX. For the purpose of this experiment, an adversary controls the input data through the API but does not have access to the weights, which remain unknown to an unprivileged user.

\input{contents/Alg}

The attack process begins with the adversary strategically manipulating the input data and observing the resulting execution times under different conditions. This timing information is then utilized to infer the values of the hidden weights. Algorithm \ref{alg:alg1} is a detailed description of the procedures used to carry out this attack.

In the fully cooled down state, running the AMX multiplier multiple times (N) highlights a clearer distinction based on the number of zeros in the operands. Accordingly, \(P1\) refers to this condition, while \(P2\) introduces a delay, allowing the AMX multiplier to cool down. Given the inherent noise in execution times, we measure these times multiple times (\(M\)) in \(P3\) to produce a less noisy composite value \(T\). This attack methodology does not impose any special precondition, and normal performance optimizations, such as turbo boost, remain enabled. In our general setup, significant timing noise arises with turbo boost active, but we mitigate these effects using differential measurements.

\paragrabf{Setting Threshold.}
By comparing execution times with inputs of full zeros and full non-zeros, we establish a differential threshold (\(Thr\)), as outlined in the algorithm \ref{alg:alg1} (Lines 1-5). This threshold enables the selective acceptance of randomly generated input vectors for scoring.The essence of the attack involves two key steps: (1) continuously generating random input vectors throughout the duration of the attack, and (2) using the execution time associated with each vector to accumulate evidence that helps refine the estimates of the weight scores.

Suppose a weight element is non-zero; then, the execution time will be longer if the corresponding input element is non-zero compared to when it is zero. Conversely, if a weight element is zero, the execution time remains unchanged whether the corresponding input element is zero or not. Based on these assumptions, if a generated input vector has a higher number of correct non-zeros according to the unknown weights, it is more likely to be accepted by this algorithm, thereby impacting the scoring tables.

\paragrabf{Execution Time Analysis and Vector Selection.}
The attacker measures the execution times for two scenarios: one for the randomly generated vector (\(W_s\)) and another for its inverted version (\(W_r\)). This is shown in lines 6-9 of Algorithm \ref{alg:alg1}. We predict that the vector holding more correct non-zeros according to the unknown weights will require a longer execution time. As shown in lines 10-15, if the difference in execution times exceeds the threshold, then either \(W_s\) or \(W_r\)—the one which records the longer time—will be selected (\(W_x\)) for updating the score vectors (\(ScoreZ\) and \(ScoreN\)). 

\paragrabf{Updating Scoring Vectors.}
After selecting \(W_x\), a scoring method updates the score vectors according to \(W_x\) entries (Lines 16-22). This involves iterating through each element of \(W_x\) from 0 to 63, incrementing the corresponding entry in \(ScoreZ\) by one if the element is zero, and in \(ScoreN\) if the element is non-zero.

\paragrabf{Inferring Weights from Scoring Vectors.}
Following the attack period, the attacker analyzes the ScoreZ and ScoreN vectors as illustrated in lines 25-31. A weight element marked as zero would be expected to yield similar scores in both \(ScoreZ\) and \(ScoreN\) vectors. However, for a weight element marked as non-zero, a higher score is expected in the \(ScoreN\) vector compared to the \(ScoreZ\).

By dividing each element of \(ScoreN\) by \(ScoreZ\), the attacker can infer the zero weights. If the ratio is close to 1, it suggests that the weight scores are equivalent and thus the weight is likely zero. A ratio significantly above 1 indicates that the weight is likely non-zero.

\paragrabf{Results Analysis.}
After extensive experiments, the configurable parameters in Algorithm \ref{alg:alg1} were selected to the following values: \(N=10000\), \(M=40\), \(L=20\), \(K=3\), \(\alpha=0.9\), and \(\gamma=1.13\), which were effective in demonstrating the outcome. Prolonging the attack duration reduces noise in the scores and enhances the success rate of accurately determining the weights. 



Figure \ref{fig:ML_SuccessRate} shows success rates increasing with longer attack durations, from 60\% at 5 minutes to a complete 100\% success rate at 50 minutes (0.02 bit/s) and beyond. Since cooling down the AMX is necessary for every timing measurement, over 99\% of the attack duration is consumed by cooling delays. Additionally, the results of the algorithm for two different attack durations are shown in Figure \ref{fig:LeakedWeights}. 







%%%%%%%%From ISCA 

\subsubsection{Instruction Reuse Dependency} \label{sec:stages}
In an experiment, we measured how long it takes to execute a single AMX multiplication instruction while varying the intervals between consecutive executions. 

% % \begin{lstlisting}[frame=single, numbers=left, caption={Pseudocode to generate Figure~\ref{fig:sleepstages}}, label={lst:ars-gadget1}]
% \begin{center}
% \begin{minipage}{0.8\linewidth}
% \centering
% \begin{lstlisting}[frame=single, numbers=left, caption={Test for Instruction Reuse Timing Dependency Detection}, label={lst:ars-gadget1}, basicstyle=\scriptsize\ttfamily, captionpos=b]
%     t = RDTSCP()
%     TDPBSSD %tmm0, %tmm1, %tmm2
%     while (RDTSCP() < t + interval_delay) {}
%     start = RDTSCP()
%     TDPBSSD %tmm3, %tmm4, %tmm5
%     end = RDTSCP()
%     report end-start
% \end{lstlisting}
% \end{minipage}
% \end{center}

% In Listing~\ref{lst:ars-gadget1}, we present the high-level pseudocode that generated Figure~\ref{fig:Performance_Stages}. In line 1, we obtain the current time using the highest available resolution timer on the platform, e.g. \texttt{RDTSCP} on x86. In line 2, we perform a \texttt{TDPBSSD} - AMX signed integer-signed integer matrix to warm up the TMUL unit. In particular, we matrix-multiply the contents of the tile register TMM0 and TMM1 and store the result in TMM2. In line 3, we wait for a particular time, doing nothing. To simulate the conditions of a typical program, we added non-AMX instructions during these intervals.  On lines 4-6, we time the execution time of a \texttt{TDPBSSD}, making sure to use different registers than the operation on line 2 to ensure that there isn't some identical operand optimization we are measuring. We finally report the time on line 7.


% \begin{figure}[!htbp]
%     \centering
%     \begin{tikzpicture}
%         \begin{axis}[
%             xmin=100, xmax=1000000000,
%             ymin=10,
%             xlabel={Interval Delay (Cycle)},
%             ylabel={Multiplication Execution\\Time (Cycle)},
%             xmode=log, 
%             ymode=log,
%             log basis x=10, 
%             log basis y=10,
%             grid=both,
%             major grid style={line width=0pt,draw=white!50},
%             minor grid style={line width=0pt,draw=white!20},
%             font=\scriptsize,
%             ylabel style={yshift=0pt, align=center}, 
%             width=\linewidth*0.8,
%             height=\linewidth*0.4,
%         ]
%             \addplot[darkgray, thick] table {Diagrams/Data/warmup.txt};
%         \end{axis}
        
%         \draw[->, black, thick] (1.1,0.39) -- (0.75,0.38) node[midway, above] {\tiny };
%          \node[black, thick] at (1.6,0.39) {\tiny Warm State};
%          \node[gray, thick] at (1.3,0.9) {\tiny Cold State 1};
%          \node[gray, thick] at (1.9,1.3) {\tiny Cold State 2};
%          \node[gray, thick] at (3.8,1.45) {\tiny Cold State 3};
%          \node[gray, thick] at (5,1.75) {\tiny Cold State 4};
         
%     \end{tikzpicture}
%     \caption{Five Distinct Performance States of
% TMUL.}
%     \label{fig:Performance_Stages}
% \end{figure}




%In Figure~\ref{fig:Performance_Stages}, w
We observe that the latency of a \texttt{TDPBSSD} (signed-signed 8-bit integer matrix multiplication) differs depending on the time since the AMX unit was last used, ie \textit{ reuse}. 
By changing the length of these intervals, we observed five distinct execution times for the AMX multiplication instruction.  We noticed that this latency goes through five distinct \textit{performance stages} which correspond to a 50, 600, 6000, 9000, and 20000 tsc latency to perform a \texttt{TDPBSSD}. We classified these into performance states, with the shortest execution time labeled as the "Warm State", the longer execution times are referred to as "Cold States" specifically Cold State 1 (the second shortest), Cold State 2, Cold State 3, and Cold State 4 (the longest).  
%Figure \ref{fig:Performance_Stages} visually represents these performance states. 

%Thus, execution time can serve as a proxy for Instruction Reuse/Utilization. 
%The methodology used here can be applied to other instructions by replacing the AMX instruction with specific operations and systematically varying the reuse intervals. 
%By varying the interval delay between successive executions of AMX instructions, a secret value can be transmitted to the attacker through time measurement, and the attacker can manipulate Intel AMX utilization through instruction reuse to bring the AMX performance state to the known state.
% \begin{tcolorbox}[
%     colback=lightgray!20,    % Light grey background
%     colframe=gray!50,        % Light gray border
%     boxrule=0.3mm,           % Thin border thickness
%     arc=2mm,                 % Slightly rounded corners
%     width=0.48\textwidth,     % Half the page width
%     sharp corners=all,
%     left=2mm,                % Adjust left padding
%     right=2mm,               % Adjust right padding
%     top=1mm,                 % Adjust top padding
%     bottom=1mm               % Adjust bottom padding
% ]
%  % {Thus, execution time can serve as a proxy for Instruction Reuse/Utilization. The methodology used here can be applied to other instructions by replacing the AMX instruction with specific operations and systematically varying reuse intervals. By varying the interval delay between successive executions of AMX instructions a secret value can be transmitted to the attacker through time measurement, and attacker can manipulate Intel AMX utilization through instruction reuse to bring the AMX performance state to the known state.}
% \end{tcolorbox}

%We hypothesize that these five stages are related to frequency scaling. Notably, this phenomenon is observable with both Intel Turbo Boost enabled and disabled. In the next steps, we will investigate that. 

%\subsection{Impact of CPU Frequency on Performance States.} 
\subsubsection{Frequency Dependency } \label{sec:frequencyDependency}
%In a supplementary experiment, 
Next, we investigated how changing the CPU frequency, using the "cpufreq" feature, affects the execution time of the previously identified performance states. For this study, we fixed the CPU frequency at various levels and measured the execution times for each performance state without allowing frequency scaling to adjust it dynamically.  
%

\begin{figure}[t!]
\centering
\begin{tikzpicture}
    \begin{axis}[
        xlabel={CPU Frequency (MHz)},
        ylabel={Execution time (RDTSCP cycle)},
        legend pos=outer north east,
        font=\scriptsize,
        xlabel style={yshift=0pt},
        ylabel style={yshift=0pt},
        width=\linewidth*0.5,
        height=\linewidth*0.6,
        ymode=log,
        log basis y=10,
        legend style={
                legend columns=1, 
                at={(1.02,0.5)}, 
                anchor=west,   
                font=\tiny,
            },
    ]
    
    \addplot[
        thick,
        mark=diamond,
        line width=1.5pt,
        mark size=3,
        color=darkgray
    ] table {Diagrams/Data/freq4.txt};
    \addlegendentry{Cold State 4};

    \addplot[
        thick,
        mark=x,
        line width=1.5pt,
        mark size=3,
        color=darkgray
    ] table {Diagrams/Data/freq3.txt};
    \addlegendentry{Cold State 3};
 
    \addplot[
        thick,
        line width=1.5pt,
        mark=triangle,
        mark size=2,
        color=darkgray
    ] table {Diagrams/Data/freq2.txt};
    \addlegendentry{Cold State 2};

    \addplot[
        thick,
        mark=star,
        line width=1.5pt,
        mark size=3,
        color=darkgray
    ] table {Diagrams/Data/freq1.txt};
    \addlegendentry{Cold State 1};
   
    \addplot[
        thick,
        line width=1.5pt,
        mark=o,
        mark size=2,
        color=red
    ] table {Diagrams/Data/freq0.txt};
    \addlegendentry{Warm State};



    \end{axis}
\end{tikzpicture}
\caption{Execution Time of AMX Multiplication Across Performance States at Varying CPU Frequencies}
\label{fig:Execution_time_vs_Freq}
\end{figure}
The results are plotted in Figure \ref{fig:Execution_time_vs_Freq}, where each data point represents a specific CPU frequency setting. The execution time was recorded using the `rdtscp` instruction, which operates with a clock frequency reference of 2 GHz. We examined frequencies ranging from 800 MHz to 2 GHz in increments of 100 MHz, and we observed two key behaviors:
\begin{itemize}%[leftmargin=*, labelsep=0.5em]
    \item \textbf{Cold States Invariance:} For all Cold States (Cold State 1 through Cold State 4), the execution time remains \textbf{invariant} regardless of CPU frequency. For example, Cold State 4 consistently shows the longest execution time across all frequencies, emphasizing its independence from the CPU clock.
    \item \textbf{Warm State Dependency:} In contrast, the execution time in the Warm State is directly proportional to the CPU frequency, with faster frequencies yielding reduced execution times. For example, at 800 MHz, the Warm-State execution time is approximately \textbf{ 2.5 times higher} than at 2 GHz.
\end{itemize}

% This result highlights the adaptive nature of Intel AMX, where execution time in Warm State aligns closely with the current CPU frequency, while Cold States exhibit no such dependency. This behavior suggests an internal frequency adjustment mechanism within AMX.

% Our findings indicate that the execution time of the AMX multiplication instruction in all Cold States is invariant with respect to changes in the current CPU frequency. 
% %In contrast, the Warm State execution time is directly proportional to the current CPU frequency.
% In contrast, in the Warm State, performance is directly proportional to the current CPU frequency.

% \begin{tcolorbox}[ colback=lightgray!20,
% colframe=gray!50,
% boxrule=0.3mm,
% arc=2mm,
% width=0.5\textwidth,
% sharp corners=all, left=2mm,
% right=2mm,
% top=1mm,
% bottom=1mm
% ] CPU frequency acts as a proxy for AMX performance in the Warm State, with execution times directly proportional to the execution time/latency.  \end{tcolorbox}








% We respectively term these stage 0, stage 1, stage 2, stage 3, and stage 4. 


%     \begin{figure}[!ht]
% \centering
%     \includegraphics[width=0.5\textwidth]{Loki_images/sleepstages_new_v2.pdf}
%     \caption{The sleep stages of AMX. By inserting a wait (x-axis) between two TDPBSSD instructions we found that the execution time of the second TDPBSSD changed based on the length of the wait. %\SMAcomments{Please do not use scientific number! }
%     }
%     \label{fig:sleepstages}
% \end{figure}


%\begin{spacing}{1}
% \begin{lstlisting}
% for(int i = 0; i < ITERS;i++) {
%   Time = __rdtscp();// Timer
%   for (int k = 0; k < i; k++)// Delay
%      junk = junk + k;
%   cooldown_delay[i] = __rdtscp() - Time; 
%   Time =  __rdtscp()
%   AMX_INSTRUCTION();//e.g_tile_dpbssd(0, 1, 2)
%   execution_time[i] = __rdtscp() - Time; }
% \end{lstlisting}
%\end{spacing}

Based on this, we hypothesize that the five performance stages are caused by Intel AMX operating on a separate clock from the CPU, and that this clock frequency adjusts depending on AMX utilization for power and energy efficiency to increase performance and also remain under the core power limit. To verify this, we performed the following test.

%\subsection{Transition Behavior of AMX Frequency to CPU Frequency in Warm State.}
%\subsubsection{On the Root Cause of Performance Stages} \label{sec:rootcause}
Based on the results presented in Figure \ref{fig:Performance_Stages}, the execution of the TMUL multiplication instruction occurs in Cold State 4 (the longest execution time) when the operation is performed for the first time or follows a period of inactivity exceeding approximately 20 ms. If subsequent AMX multiplication instructions follow closely, all will operate in the Warm State, which is common in programs with extensive matrix multiplications.
%
To test this, we further examined the execution time in the Warm State immediately after entry, over a fixed duration, across different CPU frequencies. We changed the CPU frequency and repeat the previous experiment. 
Our observations revealed that the AMX multiplication execution time undergoes a transition period before stabilizing. Closer analysis shows that these variations are related to the AMX's internal frequency adjustments. During this transition period, AMX adjusts its frequency from a lower value towards the current CPU frequency, temporarily using intermediate frequencies. To this end, we assumed that Intel AMX has a distinct clock and functions at different frequencies in each stage. To verify, we calculated such frequency by AMX throughput at each stage. We see that the stages change to where this calculated frequency becomes equal to the set frequency of the CPU which we controlled confirming our hypothesis. 


Figure \ref{fig:Freq_transition} illustrates how the AMX frequency is adjusted to align with the CPU frequency. When the CPU frequency is set to 1.2 GHz, the AMX frequency initially ramps up, briefly stabilizes at 1 GHz, and eventually reaches the target frequency of 1.2 GHz. Similarly, when the CPU frequency is fixed at 2 GHz, the AMX frequency transitions through intermediate stages, operating at 1 GHz and 1.3 GHz before stabilizing at 2 GHz. 
These findings show that Intel AMX includes a frequency management unit that controls the operating frequency of the TMUL accelerator. This unit can potentially access or create frequencies that differ from the CPU frequency as shown as the Transition Behavior of AMX Frequency to CPU Frequency in the Warm State. 
This finding is in contrast to the root cause known for AVX performance variation, known as power up/down~\cite{netspectre} which does not vary with the core frequency.
%%%END of ISCA

==> contents/conclusion.tex <==
% This paper has exposed a new vulnerability inherent to the Intel AMX architecture. The proposed attack demonstrates how the value-dependent execution time of AMX multiplications can be leveraged to infer secret information, such as zero weights of neural networks.

% Future research must prioritize the development of innovative mechanisms to mitigate the proposed threat vector introduced by AMX and similar technologies. 
%Until then, the adoption of accelerators presents a significant escalation in the ongoing battle to secure computing systems and the sensitive data they process.


==> contents/introduction.tex <==
\newpage

\IEEEPARstart{A}{s} 
computational demands continue to rise, there is a relentless drive towards optimization and advanced design methodologies. One of the latest advancements in this field is Intel's Advanced Matrix Extensions (AMX), an on-chip accelerator integrated into newer processors, starting with the 4th Gen Intel Xeon Scalable processors, known as Sapphire Rapids. Intel AMX provides specialized hardware support, markedly improving the efficiency and speed of matrix multiplications ~\cite{intel2022amx}. While Intel AMX represents a significant advancement in matrix computation and is not vulnerable to previously reported floating-point multiplication timing side-channel attacks ~\cite{7163051}, ~\cite{9218707}, our research uncovers that it inadvertently introduces new pathways for potential security vulnerabilities, particularly in the realm of side-channel attacks.

 % Traditionally, power side-channel attacks require physical access to a system to measure power consumption or electromagnetic emissions. Such attacks are less common and practical because they require a high level of access. However, Lipp et al. \cite{Lipp2021Platypus} demonstrated a method to exploit the Running Average Power Limit (RAPL) interface for power side-channel attacks without needing physical access. Although RAPL is now a privileged interface, this example shows how existing features can be repurposed for malicious intents.

% When designing new microarchitectures, overlooking security considerations can create avenues for hardware attacks. For instance, Dynamic Voltage and Frequency Scaling (DVFS), an optimization technique for power management, can paradoxically open up new attack surfaces by converting power side-channels into timing attacks. This vulnerability was exploited in Hertzbleed \cite{wang2022hertzbleed} to leak data via throttling under power limits, and in Collide+Power \cite{kogler2023collide+}, where power limits and throttling were manipulated to convert memory power side-channels into timing variations. Notably, power limit controls are usually privileged, and throttling can be mitigated by disabling Turbo Boost. As such, our work reveals a new, generic vulnerability in Intel AMX, specifically within its power and performance management mechanisms. Unlike DVFS-related vulnerabilities, our discovered vulnerability persists irrespective of DVFS states and allows for exploitation regardless of whether DVFS is on or off. Additionally, our attack does not require shared cache—unlike Collide+Power, which necessitates shared cache access to leak data.

% In this paper, we demonstrate the feasibility of exploiting this newly discovered vulnerability in neural network operations to leak sensitive information, such as sparsity of weights. Previous works in the literature have targeted neural network models to infer architectural details, inputs, and weights, often necessitating physical access for power and electromagnetic measurements \cite{236204}, \cite{Hu2020DeepSnifferAD}, \cite{wei2018know}, \cite{Xiang2019OpenDB}, \cite{Yu2020DeepEMDN} or shared cache manipulation via known cache side-channels \cite{Hong2018SecurityAO}, \cite{Liu2020GANREDGR}, \cite{244042}. Our approach is notable for not requiring either physical access or shared cache, thereby significantly lowering the bar for potential attackers.

% Specifically, we investigate the behavior of AMX multiplication, which operates in five distinct states, fluctuating between 52 to 20,000 cycles. We discovered that due to AMX frequency adjustments, the execution times of these multiplications are not consistent when AMX is transitioning between different states. Particularly, after exiting high-latency states and before stabilizing to a steady state, the execution time becomes a data-dependent process. This dependency arises because zero values in the multiplication operands influence the trend of frequency adjustments, creating exploitable timing differences.

% We demonstrate the exploitation of this side-channel vulnerability, showing that the execution time of AMX multiplications can be systematically measured to infer the sparsity of hidden weights of a neural network. In our practical example, we successfully leaked zeros in 64 hidden weights with 100\% accuracy within 50 minutes of observation.

% This paper presents several significant contributions:
% \begin{compactitem}
% \item It identifies a novel type of data-dependent timing side-channel vulnerability within the Intel AMX accelerator.

% \item It demonstrates the techniques necessary to exploit this newly discovered timing side-channel for launching attacks on neural networks. Specifically, it illustrates how to infer zero weights and determine the sparsity of neural network weights solely by measuring execution time.
% \end{compactitem}

% \textbf{Responsible disclosure.}  We reported our attack and findings to Intel. %Moreover, we are planning to open source our code. 

==> contents/reverse_engineering.tex <==



% \begin{figure}[!t]
%     \centering
%    \includegraphics[width=\linewidth] {images/AMXarch_new_v1.pdf} 
%     \caption{Intel AMX Architecture Overview}
%     \label{fig:AMX-arch}
% \end{figure}

% \subsection{Intel AMX Architecture and Instructions.}
% Intel AMX is an integrated accelerator introduced with the 4th Gen Intel Xeon Scalable processors, specifically engineered to boost the efficiency of matrix computations. %Figure~\ref{fig:AMX-arch} illustrates the Intel AMX architecture.

% AMX introduces a new set of registers and instructions. The registers in Intel AMX are known as Tiles, a new concept in Intel CPUs that provide a matrix of data registers, as opposed to the traditional vector registers seen in previous SIMD architectures like AVX-512. AMX includes 8 Tile registers, each capable of holding up to 16 rows with 64 bytes per row, amounting to a total of 1 KB per Tile. The number of rows and the number of bytes per row can be adjusted using the LDTILECFG instruction, and this configuration information is stored as metadata in a control register known as TILECFG. Once this configuration is set, AMX instructions such as load, store, and matrix multiplication will operate according to the specified dimensions for each Tile. Intel AMX instructions are synchronized with the Intel Architecture host (IA host) instruction stream, and the Tile loads and stores are coherent with the host memory \cite{Intel_Arc_Ins_Set_Extensions}.

% Tile Matrix Multiply unit (TMUL) serves as the accelerator engine for executing multiplication calculations. When using full-size Tile operands, the latency of the multiplication instruction is 52 cycles, while pipelining allows for a throughput of 16 cycles. Intel AMX supports two data types: BF16 and INT8. Consequently, it can perform 512 multiplications and 512 additions per cycle for BF16 and 1024 multiplications and 1024 additions per cycle for INT8 \cite{IntelOptRefManual}. 

% \begin{comment}
% AMX instructions utilize port 5 as their dedicated execution port. When two hyper-threads are active within a core, they compete for the same resources to execute AMX instructions.
% \end{comment}

\section{Reverse Engineering}
In this section, we share our findings on Intel AMX obtained through reverse engineering. In our investigations, we utilized a server running Red Hat Enterprise Linux release 9.3 (Plow), equipped with Linux kernel version 5.14. The server is powered by two Intel(R) Xeon(R) Gold 5420+ CPUs. 
We did not disable any hardware features or mitigations.

\textbf{Performance States Characterization.} 
In an experiment, we measured how long it takes to execute a single AMX multiplication instruction while varying the intervals between consecutive executions. To simulate the conditions of a typical program, we added non-AMX instructions during these intervals. By changing the length of these intervals, we observed five distinct execution times for the AMX multiplication instruction. We classified these into performance states, with the shortest execution time labeled as the "Warm State." The longer execution times are referred to as "Cold States," specifically Cold State 1 (the second shortest), Cold State 2, Cold State 3, and Cold State 4 (the longest).  Figure \ref{fig:Performance_Stages} visually represents these performance states. 

%\begin{figure}[!hbp]
%\centering\includegraphics[width=0.4\textwidth]{images/sleepstages_new_v2.pdf}
%\caption{Illustration of the Five Distinct Performance States of TMUL.}
%\label{fig:Performance_Stages}
%\end{figure}
%{\color{blue} Change the figure: bias, change the ylabel, and States }

\begin{figure}
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            xmin=100, xmax=1000000000,
            ymin=10, ymax=100000,
            xlabel={Interval Delay (Cycle)},
            ylabel={Multiplication Execution\\Time (Cycle)},
            xmode=log, 
            ymode=log,
            log basis x=10, 
            log basis y=10,
            grid=both,
            major grid style={line width=0pt,draw=white!50},
            minor grid style={line width=0pt,draw=white!20},
            font=\scriptsize,
            ylabel style={yshift=0pt, align=center}, 
            width=\linewidth*1,
            height=\linewidth*0.45,
        ]
            \addplot[darkgray, thick] table {Diagrams/Data/warmup.txt};
        \end{axis}
        
        \draw[->, black, thick] (2.1,0.45) -- (1.1,0.45) node[midway, above] {\scriptsize Warm State};
         \node[gray, thick] at (1.05,1.3) {\scriptsize Cold State 1};
         \node[gray, thick] at (2.8,1.7) {\scriptsize Cold State 2};
         \node[gray, thick] at (4.9,1.85) {\scriptsize Cold State 3};
         \node[gray, thick] at (6.4,2.15) {\scriptsize Cold State 4};
         
    \end{tikzpicture}
    \caption{llustration of the Five Distinct Performance States of
TMUL.}
    \label{fig:Performance_Stages}
\end{figure}

%\begin{spacing}{1}
% \begin{lstlisting}
% for(int i = 0; i < ITERS;i++) {
%   Time = __rdtscp();// Timer
%   for (int k = 0; k < i; k++)// Delay
%      junk = junk + k;
%   cooldown_delay[i] = __rdtscp() - Time; 
%   Time =  __rdtscp()
%   AMX_INSTRUCTION();//e.g_tile_dpbssd(0, 1, 2)
%   execution_time[i] = __rdtscp() - Time; }
% \end{lstlisting}
%\end{spacing}

\textbf{Impact of CPU Frequency on Performance States.} 
In a supplementary experiment, we investigated how changing the CPU frequency, using the "cpufreq" feature, affects the execution time of the previously identified performance states. For this study, we fixed the CPU frequency at various levels and measured the execution times for each performance state without allowing frequency scaling to adjust it dynamically. 

The results are plotted in Figure \ref{fig:Execution_time_vs_Freq}, where each data point represents a specific CPU frequency setting. Execution time was recorded using the `rdtscp` instruction, which operates with a 2 GHz clock frequency reference. We examined frequencies ranging from 800 MHz to 2 GHz in increments of 100 MHz.

Our findings indicate that the execution time of the AMX multiplication instruction in all Cold States is invariant with respect to changes in the current CPU frequency. In contrast, the Warm State execution time is directly proportional to the current CPU frequency.

%\begin{figure}[!hbp]
%\centering\includegraphics[width=0.4\textwidth]{images/Execution_time_vs_Freq.pdf}
%\caption{Execution Time of AMX Multiplication Across Performance States at Varying CPU Frequencies}
%\label{fig:Execution_time_vs_Freq}
%\end{figure}
%{\color{blue} Put Execution\_time\_vs\_Freq figure here}


\begin{figure}[t!]
\centering
\begin{tikzpicture}
    \begin{axis}[
        xlabel={CPU Frequency (MHz)},
        ylabel={Execution time (RDTSCP cycle)},
        legend pos=outer north east,
        font=\scriptsize,
        xlabel style={yshift=0pt},
        ylabel style={yshift=0pt},
        width=\linewidth*0.8,
        height=\linewidth*0.45,
        ymode=log,
        log basis y=10,
        legend style={
                legend columns=1, 
                at={(1.02,0.5)}, 
                anchor=west,   
                font=\tiny,
            },
    ]
    
    \addplot[
        thick,
        mark=diamond,
        line width=1.5pt,
        mark size=3,
        color=darkgray
    ] table {Diagrams/Data/freq4.txt};
    \addlegendentry{Cold State 4};

    \addplot[
        thick,
        mark=x,
        line width=1.5pt,
        mark size=3,
        color=darkgray
    ] table {Diagrams/Data/freq3.txt};
    \addlegendentry{Cold State 3};
 
    \addplot[
        thick,
        line width=1.5pt,
        mark=triangle,
        mark size=2,
        color=darkgray
    ] table {Diagrams/Data/freq2.txt};
    \addlegendentry{Cold State 2};

    \addplot[
        thick,
        mark=star,
        line width=1.5pt,
        mark size=3,
        color=darkgray
    ] table {Diagrams/Data/freq1.txt};
    \addlegendentry{Cold State 1};
   
    \addplot[
        thick,
        line width=1.5pt,
        mark=o,
        mark size=2,
        color=red
    ] table {Diagrams/Data/freq0.txt};
    \addlegendentry{Warm State};



    \end{axis}
\end{tikzpicture}
\caption{Execution Time of AMX Multiplication Across Performance States at Varying CPU Frequencies}
\label{fig:Execution_time_vs_Freq}
\end{figure}

\textbf{Transition Behavior of AMX Frequency to CPU Frequency in Warm State.}
Based on the results presented in Figure \ref{fig:Performance_Stages}, the execution of the TMUL multiplication instruction occurs in Cold State 4 (the longest execution time) when either the operation is performed for the first time or follows a period of inactivity exceeding approximately 20 ms. If subsequent AMX multiplication instructions follow closely, all will operate in the Warm State, which is common in programs with extensive matrix multiplications.

We further examined the execution time in the Warm State immediately after entry, over a fixed duration, across different CPU frequencies. Our observations revealed that the AMX multiplication execution time undergoes a transition period before stabilizing. Closer analysis shows that these variations are related to the AMX's internal frequency adjustments. During this transition period, AMX adjusts its frequency from a lower value towards the current CPU frequency, temporarily using intermediate frequencies.

Figure \ref{fig:Freq_transition} illustrates how the AMX frequency adjusts to align with the CPU frequency. When the CPU frequency is set to 1.2 GHz, the AMX frequency initially ramps up, briefly stabilizes at 1 GHz, and eventually reaches the target frequency of 1.2 GHz. Similarly, when the CPU frequency is fixed at 2 GHz, the AMX frequency transitions through intermediate stages, operating at 1 GHz and 1.3 GHz before stabilizing at 2 GHz.

These findings demonstrate that Intel AMX includes a frequency management unit that controls the operating frequency of the TMUL accelerator. This unit can potentially access or create frequencies that differ from the CPU frequency.

%\begin{figure}[!hbp]
%\centering\includegraphics[width=0.4\textwidth]{images/Freq_transition.pdf}
%\caption{Illustration of AMX Frequency Adjustment During Transition Periods: (a) shows the transition to a 1.2 GHz CPU frequency, with intermediate operation at 1 GHz; (b) demonstrates the adjustment to a 2 GHz CPU frequency, passing through 1 GHz and 1.3 GHz stages.}
%\label{fig:Freq_transition}
%\end{figure}
%{\color{blue} Put Freq\_transition figure here}

\begin{figure}[h!]
\centering
\begin{tikzpicture}
    \begin{axis}[
        xlabel={Number of Instructions},
        ylabel={Execution Time (RDTSCP cycle)},
        legend pos=outer north east,
        font=\scriptsize,
        xlabel style={yshift=5pt},
        ylabel style={yshift=-15pt},
        width=\linewidth*1,
        height=\linewidth*0.45,
        xmin= -0.1,xmax=40000,
        legend style={
                legend columns=-1,
                at={(0.5,1.16)},
                anchor=north, 
                font=\tiny,
                /tikz/column 2/.style={column sep=5pt}, 
            },
    ]
    
    \addplot[
        line width=0.8pt,
        color=black,
    ] table {Diagrams/Data/1400MHz.txt};
    \addlegendentry{1.2 GHz
CPU frequency};


    \addplot[
        line width=0.8pt,
        color=lightgray,
    ] table {Diagrams/Data/2000MHz.txt};
    \addlegendentry{2 GHz
CPU frequency};

    \end{axis}
    
    \node[darkgray, thick] at (2.7,1.57) {\scriptsize 1 GHz};
    \node[darkgray, thick] at (5.7,1.175) {\scriptsize 1.2 GHz};
    \node[darkgray, thick] at (2.5,1.01) {\scriptsize 1.3 GHz};
    \node[darkgray, thick] at (5.5,0.37) {\scriptsize 2 GHz};
\end{tikzpicture}
\caption{Illustration of AMX Frequency Adjustment During Transition Periods: The black graph depicts the transition to a 1.2 GHz CPU frequency, with intermediate operation at 1 GHz; The gray graph demonstrates the adjustment to a 2 GHz CPU frequency, passing through 1 GHz and 1.3 GHz stages.}
\label{fig:Freq_transition}
\end{figure}

\textbf{Impact of Operand Sparsity on TMUL Transition in Warm State.}
In our investigation of the TMUL execution time transition in the Warm State, we discovered an interesting effect involving zero values in the Tile operands during multiplication. By varying the number of zero values in the operands, we observed that increasing the number of zeros accelerates the transition period. This effect is illustrated in Figure \ref{fig:Effect_of_zeros_on_transition}, which presents three graphs depicting operand sparsity levels: 100\% sparsity, 50\% sparsity, and 0\% sparsity. In Figure \ref{fig:Effect_of_zeros_on_transition}, with the CPU frequency fixed at 2 GHz, the results indicate that higher operand sparsity in the Tile operands leads to faster convergence of the TMUL frequency to the CPU frequency.

%\begin{figure}[!hbp]
%\centering\includegraphics[width=0.4\textwidth]{images/Effect_of_zeros_on_transition.pdf}
%\caption{Impact of Operand Sparsity on the Transition Period of TMUL Frequency: The graphs depict the transition behavior with 100\%, 50\%, and 0\% sparsity levels in the Tile operands, showing faster convergence to the CPU frequency with increased sparsity.}
%\label{fig:Effect_of_zeros_on_transition}
%\end{figure}
%{\color{blue} Put Freq\_transition figure here}

\begin{figure}[h!]
\centering
\begin{tikzpicture}
    \begin{axis}[
        xlabel={Number of Instructions},
        ylabel={Execution Time (RDTSCP cycle)},
        legend pos=outer north east,
        font=\scriptsize,
        xlabel style={yshift=5pt},
        ylabel style={yshift=-15pt},
        width=\linewidth*1,
        height=\linewidth*0.48,
        xmin= -0.1,xmax=40000,
        legend style={
                legend columns=-1,
                at={(0.5,1.16)},
                anchor=north, 
                font=\tiny,
                /tikz/column 2/.style={column sep=5pt}, 
            },
    ]
    
    \addplot[
        line width=0.8pt,
        color=black,
    ] table {Diagrams/Data/2000_0Perc.txt};
    \addlegendentry{0\% Sparcity};


    \addplot[
        line width=0.8pt,
        color=lightgray,
    ] table {Diagrams/Data/2000_50Perc.txt};
    \addlegendentry{50\% Sparcity};


    \addplot[
        line width=0.8pt,
        color=gray,
    ] table {Diagrams/Data/2000_100Perc.txt};
    \addlegendentry{100\% Sparcity};

    \end{axis}
    
    \node[darkgray, thick] at (1.2,0.57) {\scriptsize 1.8 GHz};
    \node[darkgray, thick] at (1.9,1.95) {\scriptsize 1 GHz};
    \node[darkgray, thick] at (2,1.23) {\scriptsize 1.3 GHz};
    \node[darkgray, thick] at (5.5,0.4) {\scriptsize 2 GHz};
\end{tikzpicture}
\caption{Impact of Operand Sparsity on the Transition Period of TMUL Frequency: The graphs depict the transition behavior with 100\%, 50\%, and 0\% sparsity levels in the Tile operands, showing faster convergence to the CPU frequency with increased sparsity.}
\label{fig:Effect_of_zeros_on_transition}
\end{figure}

Consequently, the execution time of a program utilizing AMX multiplications is closely associated with the sparsity of its input operands. In Figure \ref{fig:Cumulative_execution_time}, we demonstrate this relationship by executing two test programs with 100 and 1000 AMX multiplications, each with varying Tile operand sparsity levels (0\%, 50\%, and 100\%). To construct the histogram, each scenario was executed 1,000 times. Our results reveal that varying levels of sparsity significantly impact the cumulative execution time of AMX multiplications, with increased sparsity leading to faster program execution.

This discovery uncovers a new value-dependent timing side channel that reveals the sparsity of Tile operands in Intel AMX.

% \begin{figure}[htbp!]
%     \centering
%     \begin{tikzpicture}
%         \begin{axis}[
%             font=\scriptsize,
%             width=\linewidth*0.95,
%             height=\linewidth*0.35,
%             bar width=50,
%             xmin=21800, xmax=24650,
%             xlabel={Execution time (cycle)},
%             ybar,
%             ylabel={Frequency},
%             ylabel style={yshift=-15pt},
%             ymin=0, ymax=0.006,
%             legend style={
%                 at={(0.5,1)}, 
%                 anchor=north, 
%                 legend columns=-1,
%                 font=\scriptsize,
%                 /tikz/column 2/.style={column sep=5pt}, 
%                 fill=none,
%                 draw=none
%             },
%             legend image code/.code={\draw[fill=#1,draw=none] (0cm,-0.1cm) rectangle (0.25cm,0.1cm);},
%             legend entries={100\% sparsity, 50\% sparsity, 0\% sparsity}
%         ]
%             \addplot+[hist={density, bins=50}, fill=lightgray, draw=none] table[y index=0] {Diagrams/Data/100-0.txt};
%             \addplot+[hist={density, bins=50}, fill=black, draw=none] table[y index=0] {Diagrams/Data/100-half.txt};
%             \addplot+[hist={density, bins=50}, fill=gray, draw=none] table[y index=0] {Diagrams/Data/100-1.txt};
%         \end{axis}
%         \node[anchor=south east] at (rel axis cs:-0.05,1) {(a)};
%     \end{tikzpicture}
%     \begin{tikzpicture}
%         \begin{axis}[
%             font=\scriptsize,
%             width=\linewidth*0.95,
%             height=\linewidth*0.35,
%             bar width=50,
%             xmin=35500, xmax=56000,
%             xlabel={Execution time (cycle)},
%             ybar,
%             ylabel={Frequency},
%             ylabel style={yshift=-15pt},
%             ymin=0, ymax=0.0024,
%             legend style={
%                 at={(0.5,1)}, 
%                 anchor=north, 
%                 legend columns=-1,
%                 font=\scriptsize,
%                 /tikz/column 2/.style={column sep=5pt}, 
%                 fill=none,
%                 draw=none
%             },
%             legend image code/.code={\draw[fill=#1,draw=none] (0cm,-0.1cm) rectangle (0.25cm,0.1cm);},
%             legend entries={100\% sparsity, 50\% sparsity, 0\% sparsity}
%         ]
%             \addplot+[hist={density, bins=60}, fill=lightgray, draw=none] table[y index=0] {Diagrams/Data/1000-0.txt};
%             \addplot+[hist={density, bins=60}, fill=black, draw=none] table[y index=0] {Diagrams/Data/1000-half.txt};
%             \addplot+[hist={density, bins=60}, fill=gray, draw=none] table[y index=0] {Diagrams/Data/1000-1.txt};
%         \end{axis}
%         \node[anchor=south east] at (rel axis cs:-0.05,1) {(b)};
%     \end{tikzpicture}
%     \begin{comment}
%     \begin{tikzpicture}
%         \begin{axis}[
%             font=\scriptsize,
%             width=\linewidth*0.95,
%             height=\linewidth*0.5,
%             bar width=50,
%             xmin=170000, xmax=345000,
%             xlabel={Execution time (cycle)},
%             ybar,
%             ylabel={Frequency},
%             ylabel style={yshift=-15pt},
%             ymin=0, ymax=0.00022,
%             legend style={
%                 at={(0.5,1)}, 
%                 anchor=north, 
%                 legend columns=-1,
%                 font=\scriptsize,
%                 /tikz/column 2/.style={column sep=5pt}, 
%                 fill=none,
%                 draw=none
%             },
%             legend image code/.code={\draw[fill=#1,draw=none] (0cm,-0.1cm) rectangle (0.25cm,0.1cm);},
%             legend entries={100\% sparsity, 50\% sparsity, 0\% sparsity}
%         ]
%             \addplot+[hist={density, bins=60}, fill=lightgray, draw=none] table[y index=0] {Diagrams/Data/10000-0.txt};
%             \addplot+[hist={density, bins=60}, fill=black, draw=none] table[y index=0] {Diagrams/Data/10000-half.txt};
%             \addplot+[hist={density, bins=60}, fill=gray, draw=none] table[y index=0] {Diagrams/Data/10000-1.txt};
%         \end{axis}
%         \node[anchor=south east] at (rel axis cs:-0.05,1) {(c)};
%     \end{tikzpicture}
%     \end{comment}
% \begin{comment}
% \caption{Cumulative Execution Time of Programs with Varying Operand Sparsity: The histogram illustrates the effect of operand sparsity on program execution time, highlighting that higher sparsity levels result in quicker execution across different counts of AMX multiplications. Subfigures (a), (b), and (c) represent programs with 100, 1,000, and 10,000 AMX multiplications, respectively.}
% \end{comment}
% \caption{Cumulative Execution Time of Programs with Varying Operand Sparsity: The histogram illustrates the effect of operand sparsity on program execution time, highlighting that higher sparsity levels result in quicker execution across different counts of AMX multiplications. Subfigures (a) and (b) represent programs with 100 and 1,000 AMX multiplications, respectively.}
% \label{fig:Cumulative_execution_time}
% \end{figure}


%\begin{figure}[!htbp]
%\centerline{\includegraphics[width=0.35\textwidth]{images/new_pic.pdf}}
%\caption{Cumulative Execution Time of Programs with Varying Operand Sparsity: The %histogram illustrates the effect of operand sparsity on program execution time, %highlighting that higher sparsity levels result in quicker execution across %different counts of AMX multiplications. Subfigures (a), (b), and (c) represent %programs with 100, 1,000, and 10,000 AMX multiplications, respectively.}
%\label{fig:Cumulative_execution_time}
%\end{figure}

\begin{comment}
\textbf{Operand Patterns Influencing Data-Dependent Timing in AMX Multiplications.}
In this part, we describe specific operand patterns that can accelerate the TMUL frequency transition, thereby reducing cumulative execution time. As previously mentioned, Intel AMX supports both BF16 and Int8 operand types. 

For BF16 operands, we examined both normal values and special values, including zero, subnormal, NaN, and infinity. Consider an element \( x \) in the first Tile operand being multiplied by an element \( y \) in the second Tile operand. Our findings indicate that to expedite the frequency transition, at least one of the operands \( x \) or \( y \) should be zero or subnormal, while the other should be a normal value. In Intel AMX, subnormal values are treated as zeros, meaning that if an input is subnormal, it will be considered as zero. Additionally, if an output element falls into the subnormal range, AMX returns zero for that element. Table \ref{tab:BF16Pattern} lists all possible cases for BF16 operands, highlighting those patterns that facilitate quicker transitions.



\begin{table}[ht]
    \centering
    \resizebox{0.49\textwidth}{!}{%
    \begin{tabular}{|c|c|c|c|}
        \hline
        \backslashbox{Operand 1}{Operand 2} & Normal & Zero/Subnormal & NaN/Inf \\ \hline
        Normal & - & \ding{51} & - \\ \hline
        Zero/Subnormal & \ding{51} & \ding{51} & - \\ \hline
        NaN/Inf & - & - & - \\ \hline
    \end{tabular}
    }
    \caption{BF16 Operand Patterns in Intel AMX: Cases marked with \ding{51} indicate patterns that expedite the TMUL frequency adjustment.}
\label{tab:BF16Pattern}
\end{table}

For Int8 operands, the data-dependent pattern involves zero values in two consecutive Int8 entries within a row. Specifically, this occurs in the \(2k\) and \(2k + 1\) columns of the Tiles, where \(k\) ranges from 0 to \(C/2 - 1\), with \(C\) representing the number of bytes in each row of the Tile. Suppose element \( x(r_1,2i) \) and element \( x(r_1,2i+1) \) in the first Tile are multiplied by element \( y(r_2,2j) \) and element \( y(r_2,2j+1) \) in the second Tile, respectively. Table \ref{tab:Int8Pattern} highlights the combinations of these 4 values that lead to a faster frequency transition.

\begin{table}[ht]
    \centering
    \resizebox{0.47\textwidth}{!}{%
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        \backslashbox{Operand 1}{Operand 2} & [Z, Z] & [Z, N] & [N, Z] & [N, N] \\ \hline
        {[}Z, Z{]} & \ding{51} & \ding{51} & \ding{51} & \ding{51} \\ \hline
        {[}Z, N{]} & \ding{51} & - & \ding{51} & - \\ \hline
        {[}N, Z{]} & \ding{51} & \ding{51} & - & - \\ \hline
        {[}N, N{]} & \ding{51} & - & - & - \\ \hline
    \end{tabular}
    }
    \caption{Int8 Operand Patterns: Entries marked with \ding{51} indicate patterns that accelerate TMUL frequency transition.\newline \small(Z = Zero, N = Non-zero)}
\label{tab:Int8Pattern}
\end{table}

Our results suggest the presence of a zero-skipping mechanism for both BF16 and Int8 operands. The Int8 results indicate that zero-skipping evaluates two bytes concurrently, which is likely due to the simultaneous processing of two Int8 multiplications in a specific pipeline stage within TMUL. Bypassing this pipeline stage necessitates checking both consecutive bytes. We hypothesize that bypassing these Tile element multiplications reduces AMX energy consumption, allowing the frequency management unit to increase TMUL frequency with fewer restrictions. Although the latency and throughput of AMX multiplications are fixed in terms of AMX cycles, they are influenced by operand sparsity when viewed in CPU cycles.

\end{comment}

==> contents/threats.tex <==
In MLaaS, trusted clients submit DNNs or training data to MLaaS service providers (e.g., an Amazon or Google data- center). Service providers host the DNNs, and allow remote untrusted users to submit queries to the DNNs for a fee.
